Search for $D^0$ meson decays to $\pi^+ \pi^- e^+ e^-$ and $K^+ K^- e^+ e^-$ final states

A search for $D^0$ meson decays to the $\pi^+\pi^-e^+e^-$ and $K^+K^-e^+e^-$ final states is reported using a sample of proton-proton collisions collected by the LHCb experiment at a center-of-mass energy of 13 TeV, corresponding to an integrated luminosity of 6 fb$^{-1}$. The decay $D^0 \rightarrow \pi^+\pi^-e^+e^-$ is observed for the first time when requiring that the two electrons are consistent with coming from the decay of a $\phi$ or $\rho^0/\omega$ meson. The corresponding branching fractions are measured relative to the $D^0 \rightarrow K^-\pi^-[e^+e^-]_{\rho^0/\omega}$ decay, where the two electrons are consistent with coming from the decay of a $\rho^0$ or $\omega$ meson. No evidence is found for the $D^0 \rightarrow K^+K^-e^+e^-$ decay and world-best limits are set on its branching fraction. The results are compared to, and found to be consistent with, the branching fractions of the $D^0 \rightarrow \pi^+\pi^-\mu^+\mu^-$ and $D^0 \rightarrow K^+K^-\mu^+\mu^-$ decays recently measured by LHCb and confirm lepton universality at the current precision.

==> Authorship_LHCb-PAPER-2024-047-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin{\'e}n,
T. Ackernley,
A. A.  Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
K. Akiba,
P. Albicocco,
J. Albrecht,
F. Alessio,
M. Alexander,
Z. Aliouche,
P. Alvarez Cartelle,
R. Amalric,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
A. Andreianov,
P. Andreola,
M. Andreotti,
D. Andreou,
A. Anelli,
D. Ao,
F. Archilli,
M. Argenton,
S. Arguedas Cuendis,
A. Artamonov,
M. Artuso,
E. Aslanides,
R. Ata\'{i}de Da Silva,
M. Atzeni,
B. Audurier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
A.  Balboni,
W. Baldini,
L. Balzani,
H.  Bao,
J. Baptista de Souza Leite,
C. Barbero Pretel,
M. Barbetti,
I. R. Barbosa,
R.J. Barlow,
M. Barnyakov,
S. Barsuk,
W. Barter,
J. Bartz,
J.M. Basels,
S. Bashir,
G. Bassi,
B. Batsukh,
P. B.  Battista,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
N. A.  Behling,
S. Belin,
K. Belous,
I. Belov,
I. Belyaev,
G. Benane,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
S. Bernet Andres,
A. Bertolin,
C. Betancourt,
F. Betti,
J.  Bex,
Ia. Bezshyiko,
J. Bhom,
M.S. Bieker,
N.V. Biesuz,
P. Billoir,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
V. Bocharnikov,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A.  Bohare,
A. Boldyrev,
C.S. Bolognani,
R. Bolzonella,
R. B.  Bonacci,
N. Bondar,
A. Bordelius,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
E.  Bottalico,
S.A. Bouchiba,
M.  Bovill,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
J. D. Brandenburg,
A. Brea Rodriguez,
N. Breer,
J. Brodzicka,
A. Brossa Gonzalo,
J. Brown,
D. Brundu,
E. Buchanan,
L. Buonincontri,
M.  Burgos Marcos,
A.T. Burke,
C. Burr,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
A. C.  Caillet,
R. Calabrese,
S. Calderon Ramirez,
L. Calefice,
S. Cali,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J. I. Cambon Bouzas,
P. Campana,
D.H. Campora Perez,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
S.  Cesare,
A.J. Chadwick,
I. Chahrour,
M. Charles,
Ph. Charpentier,
E.  Chatzianagnostou,
M. Chefdeville,
C. Chen,
S. Chen,
Z. Chen,
A. Chernov,
S. Chernyshenko,
X.  Chiotopoulos,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
J. Cogan,
E. Cogneras,
L. Cojocariu,
S.  Collaviti,
P. Collins,
T. Colombo,
M. Colonna,
A. Comerma-Montells,
L. Congedo,
A. Contu,
N. Cooke,
I. Corredoira ,
A. Correia,
G. Corti,
J.J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
M. Cruz Torres,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
L. Dai,
X. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
J. Daniel,
A. Danilina,
P. d'Argent,
G.  Darze,
A.  Davidson,
J.E. Davies,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
V. Dedu,
S.  Dekkers,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
J. Deng,
V. Denysenko,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
I. Diachkov,
S. Didenko,
S. Ding,
L. Dittmann,
V. Dobishuk,
A. D.  Docheva,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
A. D.  Dowling,
W. Duan,
P. Duda,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
M. M. Duras,
J.M. Durham,
O. D.  Durmus,
A. Dziurda,
A. Dzyuba,
S. Easo,
E. Eckstein,
U. Egede,
A. Egorychev,
V. Egorychev,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
J. Ellbracht,
S. Ely,
A. Ene,
J. Eschle,
S. Esen,
T. Evans,
F. Fabiano,
L.N. Falcao,
Y. Fan,
B. Fang,
L. Fantini,
M. Faria,
K.   Farmer,
D. Fazzini,
L. Felkowski,
M. Feng,
M. Feo,
A. Fernandez Casani,
M. Fernandez Gomez,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.L. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
L. F.  Foreman,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. F{\"u}hring,
Y. Fujii,
T. Fulghesu,
E. Gabriel,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B.  Ganie,
H. Gao,
R. Gao,
T.Q. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
P.  Gardner,
K. G.  Garg,
L. Garrido,
C. Gaspar,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
S. Ghizzo,
Z. Ghorbanimoghaddam,
L. Giambastiani,
F. I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
L. Girardey,
C. Giugliano,
M.A. Giza,
E.L. Gkougkousis,
F.C. Glaser,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
S. Gomez Fernandez,
W.  Gomulka,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
J. A. Gooding,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
L. Grazette,
G. Graziani,
A. T. Grecu,
L.M. Greeven,
N.A. Grieser,
L. Grillo,
S. Gromov,
C.  Gu,
M. Guarise,
L.  Guerry,
V. Guliaeva,
P. A. G{\"u}nther,
A.-K. Guseinov,
E. Gushchin,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
G.  Hallett,
M.M. Halvorsen,
P.M. Hamilton,
J. Hammerich,
Q. Han,
X. Han,
S. Hansmann-Menzemer,
L. Hao,
N. Harnew,
T. H.  Harris,
M. Hartmann,
S. Hashmi,
J. He,
F. Hemmer,
C. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A. Hicheur,
G. Hijano Mendizabal,
J. Horswill,
R. Hou,
Y. Hou,
N. Howarth,
J. Hu,
W. Hu,
X. Hu,
W. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Iniukhin,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
E. Jiang,
X. Jiang,
Y. Jiang,
Y. J.  Jiang,
M. John,
A.  John Rubesh Rajan,
D. Johnson,
C.R. Jones,
T.P. Jones,
S. Joshi,
B. Jost,
J.  Juan Castella,
N. Jurik,
I. Juszczak,
D. Kaminaris,
S. Kandybei,
M.  Kane,
Y. Kang,
C. Kar,
M. Karacson,
D. Karpenkov,
A. Kauniskangas,
J.W. Kautz,
M.K. Kazanecki,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
G. Khreich,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
N. Kleijne,
K. Klimaszewski,
M.R. Kmiec,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kopciewicz,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
M. Kreps,
P. Krokovny,
W. Krupa,
W. Krzemien,
O. Kshyvanskyi,
S. Kubis,
M. Kucharczyk,
V. Kudryavtsev,
E. Kulikova,
A. Kupsc,
B. K.  Kutsenko,
D. Lacarrere,
P.  Laguarta Gonzalez,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
J.J. Lane,
R. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
H.  Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
E. D. Lesser,
B. Leverington,
A. Li,
C.  Li,
H. Li,
K. Li,
L. Li,
M. Li,
P. Li,
P.-R. Li,
Q.  Li,
S. Li,
T. Li,
T. Li,
Y. Li,
Y. Li,
Z. Lian,
X. Liang,
S. Libralon,
C. Lin,
T. Lin,
R. Lindner,
H.  Linton,
V. Lisovskyi,
R. Litvinov,
F. L.  Liu,
G. Liu,
K. Liu,
S. Liu,
W.  Liu,
Y. Liu,
Y. Liu,
Y. L.  Liu,
G. Loachamin Ordonez,
A. Lobo Salvia,
A. Loi,
T. Long,
J.H. Lopes,
A. Lopez Huertas,
S. L{\'o}pez Soli{\~n}o,
Q. Lu,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
K. Lynch,
X.-R. Lyu,
G. M.  Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B.  Mack,
I. Mackay,
L. M.  Mackey,
L.R. Madhan Mohan,
M. J.  Madurai,
A. Maevskiy,
D. Magdalinski,
D. Maisuzenko,
J.J. Malczewski,
S. Malde,
L. Malentacca,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
C. Mancuso,
R. Manera Escalero,
F. M.  Manganella,
D. Manuzzi,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
E. Mariani,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
L.  Martel,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D.  Martinez Gomez,
D. Martinez Santos,
F. Martinez Vidal,
A.  Martorell i Granollers,
A. Massafferri,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
J. Mazorra de Cos,
M. Mazurek,
M. McCann,
T.H. McGrath,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
G. Meier,
D. Melnychuk,
F. M.  Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
T. Miralles,
B. Mitreska,
D.S. Mitzel,
A. Modak,
L. Moeser,
R.A. Mohammed,
R.D. Moise,
S. Mokhnenko,
E. F. Molina Cardenas,
T. Momb{\"a}cher,
M. Monk,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
J. Moron,
W.  Morren,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
Z. M.  Mu,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M{\"u}ller,
F. Mu{\~n}oz-Rojas,
R. Murta,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
P. Neustroev,
J. Nicolini,
D. Nicotra,
E.M. Niel,
N. Nikitin,
Q. Niu,
P. Nogarolli,
P. Nogga,
C. Normand,
J. Novoa Fernandez,
G. Nowak,
C. Nunez,
H. N.  Nur,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
S. Okamura,
A. Okhotnikov,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
M. Olocco,
C.J.G. Onderwater,
R.H. O'Neil,
D. Osthues,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
O. Ozcelik,
F. Paciolla,
A.  Padee,
K.O. Padeken,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
X.  Pan,
G. Panshin,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
D.  Parmar,
B. Passalacqua,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A.  Paul,
C.J. Pawley,
A. Pellegrino,
J.  Peng,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
H.  Pereira Da Costa,
A. Pereiro Castro,
P. Perret,
A.  Perrevoort,
A. Perro,
M.J. Peters,
K. Petridis,
A. Petrolini,
J. P.  Pfaller,
H. Pham,
L. Pica,
M. Piccini,
L.  Piccolo,
B. Pietrzyk,
G. Pietrzyk,
R. N, Pilato,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V. Placinta,
M. Plo Casasus,
T. Poeschl,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
S. Poslavskii,
K. Prasanth,
C. Prouve,
D. Provenzano,
V. Pugatch,
G. Punzi,
S.  Qasim,
Q. Q.  Qian,
W. Qian,
N. Qin,
S. Qu,
R. Quagliani,
R.I. Rabadan Trejo,
J.H. Rademacker,
M. Rama,
M.  Ram\'{i}rez Garc\'{i}a,
V. Ramos De Oliveira,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
R. Ribatti,
G. R.  Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
A. Rodriguez Alvarez,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
J. Roensch,
A. Rogachev,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
V. Romanovskiy,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
M. Rotondo,
S. R.  Roy,
M.S. Rudolph,
M. Ruiz Diaz,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J. J. Saavedra-Arias,
J.J. Saborido Silva,
R. Sadek,
N. Sagidova,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
D. Saranin,
A. Sarnatskiy,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
F. Sborzacchi,
L.G. Scantlebury Smead,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
S. Schulte,
M.H. Schune,
R. Schwemmer,
G. Schwering,
B. Sciascia,
A. Sciuccati,
I. Segal,
S. Sellam,
A. Semennikov,
T. Senger,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
Y. Shang,
D.M. Shangase,
M. Shapkin,
R. S.  Sharma,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
B. Shi,
Q. Shi,
Y. Shimizu,
E. Shmanin,
R. Shorkin,
J.D. Shupperd,
R. Silva Coutinho,
G. Simi,
S. Simone,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
J.C. Smallwood,
E. Smith,
K. Smith,
M. Smith,
A. Snoch,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
A. Solovev,
I. Solovyev,
N. S.  Sommerfeld,
R. Song,
Y. Song,
Y. Song,
Y. S.  Song,
F.L. Souza De Almeida,
B. Souza De Paula,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
E. Spiridenkov,
P. Spradlin,
V. Sriskaran,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
M.  Stefaniak,
E.N. Stein,
O. Steinkamp,
O. Stenyakin,
H. Stevens,
D. Strekalina,
Y. Su,
F. Suljik,
J. Sun,
L. Sun,
D. Sundfeld,
W. Sutcliffe,
P.N. Swallow,
K. Swientek,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
Y. Tang,
M.D. Tat,
A. Terentev,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
L. Tomassetti,
G. Tonani,
X. Tong,
T. Tork,
D. Torres Machado,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
D.J. Unverzagt,
B.  Urbach,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
V. Vagnoni,
V.  Valcarce Cadenas,
G. Valenti,
N. Valls Canudas,
J. van Eldik,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
G. Vasquez,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Verdoglia,
M. Vesterinen,
D.  Vico Benet,
P.  Vidrier Villalba,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
F.C. Volle,
D. vom Bruch,
N. Voropaev,
K. Vos,
C. Vrahas,
J. Wagner,
J. Walsh,
E.J. Walton,
G. Wan,
C. Wang,
G. Wang,
H. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N. W.  Wang,
R. Wang,
X. Wang,
X. Wang,
X. W.  Wang,
Y. Wang,
Y. W.  Wang,
Z. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
J. Wendel,
B.D.C. Westhenry,
C. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M. J. Williams,
M.R.J. Williams,
R. Williams,
Z.  Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
L. Witola,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
X. Wu,
Y. Wu,
Z. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
T. X.  Xing,
A. Xu,
L. Xu,
L. Xu,
M. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
K.  Yang,
S. Yang,
X. Yang,
Y. Yang,
Z. Yang,
V. Yeroshenko,
H. Yeung,
H. Yin,
X.  Yin,
C. Y.  Yu,
J. Yu,
X. Yuan,
Y Yuan,
E. Zaffaroni,
M. Zavertyaev,
M. Zdybal,
F. Zenesini,
C.  Zeng,
M. Zeng,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
S. Zhang,
S. Zhang,
Y. Zhang,
Y. Z.  Zhang,
Z. Zhang,
Y. Zhao,
A. Zhelezov,
S. Z.  Zheng,
X. Z.  Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
L. Z.  Zhu,
X. Zhu,
X. Zhu,
V. Zhukov,
J. Zhuo,
Q. Zou,
D. Zuliani,
G. Zunica

==> Authorship_LHCb-PAPER-2024-047.tex <==
% LHCb collaboration author list
% Data extracted on December 6th, 2024 at 9:49am for paper reference LHCb-PAPER-2024-047
\centerline
{\large\bf LHCb collaboration}
\begin
{flushleft}
\small
R.~Aaij$^{38}$\lhcborcid{0000-0003-0533-1952},
A.S.W.~Abdelmotteleb$^{57}$\lhcborcid{0000-0001-7905-0542},
C.~Abellan~Beteta$^{51}$,
F.~Abudin{\'e}n$^{57}$\lhcborcid{0000-0002-6737-3528},
T.~Ackernley$^{61}$\lhcborcid{0000-0002-5951-3498},
A. A. ~Adefisoye$^{69}$\lhcborcid{0000-0003-2448-1550},
B.~Adeva$^{47}$\lhcborcid{0000-0001-9756-3712},
M.~Adinolfi$^{55}$\lhcborcid{0000-0002-1326-1264},
P.~Adlarson$^{82}$\lhcborcid{0000-0001-6280-3851},
C.~Agapopoulou$^{14}$\lhcborcid{0000-0002-2368-0147},
C.A.~Aidala$^{83}$\lhcborcid{0000-0001-9540-4988},
Z.~Ajaltouni$^{11}$,
S.~Akar$^{11}$\lhcborcid{0000-0003-0288-9694},
K.~Akiba$^{38}$\lhcborcid{0000-0002-6736-471X},
P.~Albicocco$^{28}$\lhcborcid{0000-0001-6430-1038},
J.~Albrecht$^{19,f}$\lhcborcid{0000-0001-8636-1621},
F.~Alessio$^{49}$\lhcborcid{0000-0001-5317-1098},
M.~Alexander$^{60}$\lhcborcid{0000-0002-8148-2392},
Z.~Aliouche$^{63}$\lhcborcid{0000-0003-0897-4160},
P.~Alvarez~Cartelle$^{56}$\lhcborcid{0000-0003-1652-2834},
R.~Amalric$^{16}$\lhcborcid{0000-0003-4595-2729},
S.~Amato$^{3}$\lhcborcid{0000-0002-3277-0662},
J.L.~Amey$^{55}$\lhcborcid{0000-0002-2597-3808},
Y.~Amhis$^{14}$\lhcborcid{0000-0003-4282-1512},
L.~An$^{6}$\lhcborcid{0000-0002-3274-5627},
L.~Anderlini$^{27}$\lhcborcid{0000-0001-6808-2418},
M.~Andersson$^{51}$\lhcborcid{0000-0003-3594-9163},
A.~Andreianov$^{44}$\lhcborcid{0000-0002-6273-0506},
P.~Andreola$^{51}$\lhcborcid{0000-0002-3923-431X},
M.~Andreotti$^{26}$\lhcborcid{0000-0003-2918-1311},
D.~Andreou$^{69}$\lhcborcid{0000-0001-6288-0558},
A.~Anelli$^{31,o,49}$\lhcborcid{0000-0002-6191-934X},
D.~Ao$^{7}$\lhcborcid{0000-0003-1647-4238},
F.~Archilli$^{37,u}$\lhcborcid{0000-0002-1779-6813},
M.~Argenton$^{26}$\lhcborcid{0009-0006-3169-0077},
S.~Arguedas~Cuendis$^{9,49}$\lhcborcid{0000-0003-4234-7005},
A.~Artamonov$^{44}$\lhcborcid{0000-0002-2785-2233},
M.~Artuso$^{69}$\lhcborcid{0000-0002-5991-7273},
E.~Aslanides$^{13}$\lhcborcid{0000-0003-3286-683X},
R.~Ata\'{i}de~Da~Silva$^{50}$\lhcborcid{0009-0005-1667-2666},
M.~Atzeni$^{65}$\lhcborcid{0000-0002-3208-3336},
B.~Audurier$^{12}$\lhcborcid{0000-0001-9090-4254},
D.~Bacher$^{64}$\lhcborcid{0000-0002-1249-367X},
I.~Bachiller~Perea$^{10}$\lhcborcid{0000-0002-3721-4876},
S.~Bachmann$^{22}$\lhcborcid{0000-0002-1186-3894},
M.~Bachmayer$^{50}$\lhcborcid{0000-0001-5996-2747},
J.J.~Back$^{57}$\lhcborcid{0000-0001-7791-4490},
P.~Baladron~Rodriguez$^{47}$\lhcborcid{0000-0003-4240-2094},
V.~Balagura$^{15}$\lhcborcid{0000-0002-1611-7188},
A. ~Balboni$^{26}$\lhcborcid{0009-0003-8872-976X},
W.~Baldini$^{26}$\lhcborcid{0000-0001-7658-8777},
L.~Balzani$^{19}$\lhcborcid{0009-0006-5241-1452},
H. ~Bao$^{7}$\lhcborcid{0009-0002-7027-021X},
J.~Baptista~de~Souza~Leite$^{61}$\lhcborcid{0000-0002-4442-5372},
C.~Barbero~Pretel$^{47,12}$\lhcborcid{0009-0001-1805-6219},
M.~Barbetti$^{27}$\lhcborcid{0000-0002-6704-6914},
I. R.~Barbosa$^{70}$\lhcborcid{0000-0002-3226-8672},
R.J.~Barlow$^{63}$\lhcborcid{0000-0002-8295-8612},
M.~Barnyakov$^{25}$\lhcborcid{0009-0000-0102-0482},
S.~Barsuk$^{14}$\lhcborcid{0000-0002-0898-6551},
W.~Barter$^{59}$\lhcborcid{0000-0002-9264-4799},
J.~Bartz$^{69}$\lhcborcid{0000-0002-2646-4124},
J.M.~Basels$^{17}$\lhcborcid{0000-0001-5860-8770},
S.~Bashir$^{40}$\lhcborcid{0000-0001-9861-8922},
G.~Bassi$^{35,r}$\lhcborcid{0000-0002-2145-3805},
B.~Batsukh$^{5}$\lhcborcid{0000-0003-1020-2549},
P. B. ~Battista$^{14}$,
A.~Bay$^{50}$\lhcborcid{0000-0002-4862-9399},
A.~Beck$^{65}$\lhcborcid{0000-0003-4872-1213},
M.~Becker$^{19}$\lhcborcid{0000-0002-7972-8760},
F.~Bedeschi$^{35}$\lhcborcid{0000-0002-8315-2119},
I.B.~Bediaga$^{2}$\lhcborcid{0000-0001-7806-5283},
N. A. ~Behling$^{19}$\lhcborcid{0000-0003-4750-7872},
S.~Belin$^{47}$\lhcborcid{0000-0001-7154-1304},
K.~Belous$^{44}$\lhcborcid{0000-0003-0014-2589},
I.~Belov$^{29}$\lhcborcid{0000-0003-1699-9202},
I.~Belyaev$^{36}$\lhcborcid{0000-0002-7458-7030},
G.~Benane$^{13}$\lhcborcid{0000-0002-8176-8315},
G.~Bencivenni$^{28}$\lhcborcid{0000-0002-5107-0610},
E.~Ben-Haim$^{16}$\lhcborcid{0000-0002-9510-8414},
A.~Berezhnoy$^{44}$\lhcborcid{0000-0002-4431-7582},
R.~Bernet$^{51}$\lhcborcid{0000-0002-4856-8063},
S.~Bernet~Andres$^{45}$\lhcborcid{0000-0002-4515-7541},
A.~Bertolin$^{33}$\lhcborcid{0000-0003-1393-4315},
C.~Betancourt$^{51}$\lhcborcid{0000-0001-9886-7427},
F.~Betti$^{59}$\lhcborcid{0000-0002-2395-235X},
J. ~Bex$^{56}$\lhcborcid{0000-0002-2856-8074},
Ia.~Bezshyiko$^{51}$\lhcborcid{0000-0002-4315-6414},
J.~Bhom$^{41}$\lhcborcid{0000-0002-9709-903X},
M.S.~Bieker$^{19}$\lhcborcid{0000-0001-7113-7862},
N.V.~Biesuz$^{26}$\lhcborcid{0000-0003-3004-0946},
P.~Billoir$^{16}$\lhcborcid{0000-0001-5433-9876},
A.~Biolchini$^{38}$\lhcborcid{0000-0001-6064-9993},
M.~Birch$^{62}$\lhcborcid{0000-0001-9157-4461},
F.C.R.~Bishop$^{10}$\lhcborcid{0000-0002-0023-3897},
A.~Bitadze$^{63}$\lhcborcid{0000-0001-7979-1092},
A.~Bizzeti$^{}$\lhcborcid{0000-0001-5729-5530},
T.~Blake$^{57}$\lhcborcid{0000-0002-0259-5891},
F.~Blanc$^{50}$\lhcborcid{0000-0001-5775-3132},
J.E.~Blank$^{19}$\lhcborcid{0000-0002-6546-5605},
S.~Blusk$^{69}$\lhcborcid{0000-0001-9170-684X},
V.~Bocharnikov$^{44}$\lhcborcid{0000-0003-1048-7732},
J.A.~Boelhauve$^{19}$\lhcborcid{0000-0002-3543-9959},
O.~Boente~Garcia$^{15}$\lhcborcid{0000-0003-0261-8085},
T.~Boettcher$^{66}$\lhcborcid{0000-0002-2439-9955},
A. ~Bohare$^{59}$\lhcborcid{0000-0003-1077-8046},
A.~Boldyrev$^{44}$\lhcborcid{0000-0002-7872-6819},
C.S.~Bolognani$^{79}$\lhcborcid{0000-0003-3752-6789},
R.~Bolzonella$^{26,l}$\lhcborcid{0000-0002-0055-0577},
R. B. ~Bonacci$^{1}$\lhcborcid{0009-0004-1871-2417},
N.~Bondar$^{44}$\lhcborcid{0000-0003-2714-9879},
A.~Bordelius$^{49}$\lhcborcid{0009-0002-3529-8524},
F.~Borgato$^{33,p}$\lhcborcid{0000-0002-3149-6710},
S.~Borghi$^{63}$\lhcborcid{0000-0001-5135-1511},
M.~Borsato$^{31,o}$\lhcborcid{0000-0001-5760-2924},
J.T.~Borsuk$^{41}$\lhcborcid{0000-0002-9065-9030},
E. ~Bottalico$^{61}$\lhcborcid{0000-0003-2238-8803},
S.A.~Bouchiba$^{50}$\lhcborcid{0000-0002-0044-6470},
M. ~Bovill$^{64}$\lhcborcid{0009-0006-2494-8287},
T.J.V.~Bowcock$^{61}$\lhcborcid{0000-0002-3505-6915},
A.~Boyer$^{49}$\lhcborcid{0000-0002-9909-0186},
C.~Bozzi$^{26}$\lhcborcid{0000-0001-6782-3982},
J. D.~Brandenburg$^{84}$\lhcborcid{0000-0002-6327-5947},
A.~Brea~Rodriguez$^{50}$\lhcborcid{0000-0001-5650-445X},
N.~Breer$^{19}$\lhcborcid{0000-0003-0307-3662},
J.~Brodzicka$^{41}$\lhcborcid{0000-0002-8556-0597},
A.~Brossa~Gonzalo$^{47,\dagger}$\lhcborcid{0000-0002-4442-1048},
J.~Brown$^{61}$\lhcborcid{0000-0001-9846-9672},
D.~Brundu$^{32}$\lhcborcid{0000-0003-4457-5896},
E.~Buchanan$^{59}$,
L.~Buonincontri$^{33,p}$\lhcborcid{0000-0002-1480-454X},
M. ~Burgos~Marcos$^{79}$\lhcborcid{0009-0001-9716-0793},
A.T.~Burke$^{63}$\lhcborcid{0000-0003-0243-0517},
C.~Burr$^{49}$\lhcborcid{0000-0002-5155-1094},
J.S.~Butter$^{56}$\lhcborcid{0000-0002-1816-536X},
J.~Buytaert$^{49}$\lhcborcid{0000-0002-7958-6790},
W.~Byczynski$^{49}$\lhcborcid{0009-0008-0187-3395},
S.~Cadeddu$^{32}$\lhcborcid{0000-0002-7763-500X},
H.~Cai$^{74}$,
A. C. ~Caillet$^{16}$,
R.~Calabrese$^{26,l}$\lhcborcid{0000-0002-1354-5400},
S.~Calderon~Ramirez$^{9}$\lhcborcid{0000-0001-9993-4388},
L.~Calefice$^{46}$\lhcborcid{0000-0001-6401-1583},
S.~Cali$^{28}$\lhcborcid{0000-0001-9056-0711},
M.~Calvi$^{31,o}$\lhcborcid{0000-0002-8797-1357},
M.~Calvo~Gomez$^{45}$\lhcborcid{0000-0001-5588-1448},
P.~Camargo~Magalhaes$^{2,z}$\lhcborcid{0000-0003-3641-8110},
J. I.~Cambon~Bouzas$^{47}$\lhcborcid{0000-0002-2952-3118},
P.~Campana$^{28}$\lhcborcid{0000-0001-8233-1951},
D.H.~Campora~Perez$^{79}$\lhcborcid{0000-0001-8998-9975},
A.F.~Campoverde~Quezada$^{7}$\lhcborcid{0000-0003-1968-1216},
S.~Capelli$^{31}$\lhcborcid{0000-0002-8444-4498},
L.~Capriotti$^{26}$\lhcborcid{0000-0003-4899-0587},
R.~Caravaca-Mora$^{9}$\lhcborcid{0000-0001-8010-0447},
A.~Carbone$^{25,j}$\lhcborcid{0000-0002-7045-2243},
L.~Carcedo~Salgado$^{47}$\lhcborcid{0000-0003-3101-3528},
R.~Cardinale$^{29,m}$\lhcborcid{0000-0002-7835-7638},
A.~Cardini$^{32}$\lhcborcid{0000-0002-6649-0298},
P.~Carniti$^{31,o}$\lhcborcid{0000-0002-7820-2732},
L.~Carus$^{22}$,
A.~Casais~Vidal$^{65}$\lhcborcid{0000-0003-0469-2588},
R.~Caspary$^{22}$\lhcborcid{0000-0002-1449-1619},
G.~Casse$^{61}$\lhcborcid{0000-0002-8516-237X},
M.~Cattaneo$^{49}$\lhcborcid{0000-0001-7707-169X},
G.~Cavallero$^{26,49}$\lhcborcid{0000-0002-8342-7047},
V.~Cavallini$^{26,l}$\lhcborcid{0000-0001-7601-129X},
S.~Celani$^{22}$\lhcborcid{0000-0003-4715-7622},
S. ~Cesare$^{30,n}$\lhcborcid{0000-0003-0886-7111},
A.J.~Chadwick$^{61}$\lhcborcid{0000-0003-3537-9404},
I.~Chahrour$^{83}$\lhcborcid{0000-0002-1472-0987},
M.~Charles$^{16}$\lhcborcid{0000-0003-4795-498X},
Ph.~Charpentier$^{49}$\lhcborcid{0000-0001-9295-8635},
E. ~Chatzianagnostou$^{38}$\lhcborcid{0009-0009-3781-1820},
M.~Chefdeville$^{10}$\lhcborcid{0000-0002-6553-6493},
C.~Chen$^{13}$\lhcborcid{0000-0002-3400-5489},
S.~Chen$^{5}$\lhcborcid{0000-0002-8647-1828},
Z.~Chen$^{7}$\lhcborcid{0000-0002-0215-7269},
A.~Chernov$^{41}$\lhcborcid{0000-0003-0232-6808},
S.~Chernyshenko$^{53}$\lhcborcid{0000-0002-2546-6080},
X. ~Chiotopoulos$^{79}$\lhcborcid{0009-0006-5762-6559},
V.~Chobanova$^{81}$\lhcborcid{0000-0002-1353-6002},
M.~Chrzaszcz$^{41}$\lhcborcid{0000-0001-7901-8710},
A.~Chubykin$^{44}$\lhcborcid{0000-0003-1061-9643},
V.~Chulikov$^{28,36}$\lhcborcid{0000-0002-7767-9117},
P.~Ciambrone$^{28}$\lhcborcid{0000-0003-0253-9846},
X.~Cid~Vidal$^{47}$\lhcborcid{0000-0002-0468-541X},
G.~Ciezarek$^{49}$\lhcborcid{0000-0003-1002-8368},
P.~Cifra$^{49}$\lhcborcid{0000-0003-3068-7029},
P.E.L.~Clarke$^{59}$\lhcborcid{0000-0003-3746-0732},
M.~Clemencic$^{49}$\lhcborcid{0000-0003-1710-6824},
H.V.~Cliff$^{56}$\lhcborcid{0000-0003-0531-0916},
J.~Closier$^{49}$\lhcborcid{0000-0002-0228-9130},
C.~Cocha~Toapaxi$^{22}$\lhcborcid{0000-0001-5812-8611},
V.~Coco$^{49}$\lhcborcid{0000-0002-5310-6808},
J.~Cogan$^{13}$\lhcborcid{0000-0001-7194-7566},
E.~Cogneras$^{11}$\lhcborcid{0000-0002-8933-9427},
L.~Cojocariu$^{43}$\lhcborcid{0000-0002-1281-5923},
S. ~Collaviti$^{50}$\lhcborcid{0009-0003-7280-8236},
P.~Collins$^{49}$\lhcborcid{0000-0003-1437-4022},
T.~Colombo$^{49}$\lhcborcid{0000-0002-9617-9687},
M.~Colonna$^{19}$\lhcborcid{0009-0000-1704-4139},
A.~Comerma-Montells$^{46}$\lhcborcid{0000-0002-8980-6048},
L.~Congedo$^{24}$\lhcborcid{0000-0003-4536-4644},
A.~Contu$^{32}$\lhcborcid{0000-0002-3545-2969},
N.~Cooke$^{60}$\lhcborcid{0000-0002-4179-3700},
I.~Corredoira~$^{47}$\lhcborcid{0000-0002-6089-0899},
A.~Correia$^{16}$\lhcborcid{0000-0002-6483-8596},
G.~Corti$^{49}$\lhcborcid{0000-0003-2857-4471},
J.J.~Cottee~Meldrum$^{55}$,
B.~Couturier$^{49}$\lhcborcid{0000-0001-6749-1033},
D.C.~Craik$^{51}$\lhcborcid{0000-0002-3684-1560},
M.~Cruz~Torres$^{2,g}$\lhcborcid{0000-0003-2607-131X},
E.~Curras~Rivera$^{50}$\lhcborcid{0000-0002-6555-0340},
R.~Currie$^{59}$\lhcborcid{0000-0002-0166-9529},
C.L.~Da~Silva$^{68}$\lhcborcid{0000-0003-4106-8258},
S.~Dadabaev$^{44}$\lhcborcid{0000-0002-0093-3244},
L.~Dai$^{71}$\lhcborcid{0000-0002-4070-4729},
X.~Dai$^{4}$\lhcborcid{0000-0003-3395-7151},
E.~Dall'Occo$^{49}$\lhcborcid{0000-0001-9313-4021},
J.~Dalseno$^{47}$\lhcborcid{0000-0003-3288-4683},
C.~D'Ambrosio$^{49}$\lhcborcid{0000-0003-4344-9994},
J.~Daniel$^{11}$\lhcborcid{0000-0002-9022-4264},
A.~Danilina$^{44}$\lhcborcid{0000-0003-3121-2164},
P.~d'Argent$^{24}$\lhcborcid{0000-0003-2380-8355},
G. ~Darze$^{3}$,
A. ~Davidson$^{57}$\lhcborcid{0009-0002-0647-2028},
J.E.~Davies$^{63}$\lhcborcid{0000-0002-5382-8683},
O.~De~Aguiar~Francisco$^{63}$\lhcborcid{0000-0003-2735-678X},
C.~De~Angelis$^{32,k}$\lhcborcid{0009-0005-5033-5866},
F.~De~Benedetti$^{49}$\lhcborcid{0000-0002-7960-3116},
J.~de~Boer$^{38}$\lhcborcid{0000-0002-6084-4294},
K.~De~Bruyn$^{78}$\lhcborcid{0000-0002-0615-4399},
S.~De~Capua$^{63}$\lhcborcid{0000-0002-6285-9596},
M.~De~Cian$^{22}$\lhcborcid{0000-0002-1268-9621},
U.~De~Freitas~Carneiro~Da~Graca$^{2,a}$\lhcborcid{0000-0003-0451-4028},
E.~De~Lucia$^{28}$\lhcborcid{0000-0003-0793-0844},
J.M.~De~Miranda$^{2}$\lhcborcid{0009-0003-2505-7337},
L.~De~Paula$^{3}$\lhcborcid{0000-0002-4984-7734},
M.~De~Serio$^{24,h}$\lhcborcid{0000-0003-4915-7933},
P.~De~Simone$^{28}$\lhcborcid{0000-0001-9392-2079},
F.~De~Vellis$^{19}$\lhcborcid{0000-0001-7596-5091},
J.A.~de~Vries$^{79}$\lhcborcid{0000-0003-4712-9816},
F.~Debernardis$^{24}$\lhcborcid{0009-0001-5383-4899},
D.~Decamp$^{10}$\lhcborcid{0000-0001-9643-6762},
V.~Dedu$^{13}$\lhcborcid{0000-0001-5672-8672},
S. ~Dekkers$^{1}$\lhcborcid{0000-0001-9598-875X},
L.~Del~Buono$^{16}$\lhcborcid{0000-0003-4774-2194},
B.~Delaney$^{65}$\lhcborcid{0009-0007-6371-8035},
H.-P.~Dembinski$^{19}$\lhcborcid{0000-0003-3337-3850},
J.~Deng$^{8}$\lhcborcid{0000-0002-4395-3616},
V.~Denysenko$^{51}$\lhcborcid{0000-0002-0455-5404},
O.~Deschamps$^{11}$\lhcborcid{0000-0002-7047-6042},
F.~Dettori$^{32,k}$\lhcborcid{0000-0003-0256-8663},
B.~Dey$^{77}$\lhcborcid{0000-0002-4563-5806},
P.~Di~Nezza$^{28}$\lhcborcid{0000-0003-4894-6762},
I.~Diachkov$^{44}$\lhcborcid{0000-0001-5222-5293},
S.~Didenko$^{44}$\lhcborcid{0000-0001-5671-5863},
S.~Ding$^{69}$\lhcborcid{0000-0002-5946-581X},
L.~Dittmann$^{22}$\lhcborcid{0009-0000-0510-0252},
V.~Dobishuk$^{53}$\lhcborcid{0000-0001-9004-3255},
A. D. ~Docheva$^{60}$\lhcborcid{0000-0002-7680-4043},
C.~Dong$^{4,b}$\lhcborcid{0000-0003-3259-6323},
A.M.~Donohoe$^{23}$\lhcborcid{0000-0002-4438-3950},
F.~Dordei$^{32}$\lhcborcid{0000-0002-2571-5067},
A.C.~dos~Reis$^{2}$\lhcborcid{0000-0001-7517-8418},
A. D. ~Dowling$^{69}$\lhcborcid{0009-0007-1406-3343},
W.~Duan$^{72}$\lhcborcid{0000-0003-1765-9939},
P.~Duda$^{80}$\lhcborcid{0000-0003-4043-7963},
M.W.~Dudek$^{41}$\lhcborcid{0000-0003-3939-3262},
L.~Dufour$^{49}$\lhcborcid{0000-0002-3924-2774},
V.~Duk$^{34}$\lhcborcid{0000-0001-6440-0087},
P.~Durante$^{49}$\lhcborcid{0000-0002-1204-2270},
M. M.~Duras$^{80}$\lhcborcid{0000-0002-4153-5293},
J.M.~Durham$^{68}$\lhcborcid{0000-0002-5831-3398},
O. D. ~Durmus$^{77}$\lhcborcid{0000-0002-8161-7832},
A.~Dziurda$^{41}$\lhcborcid{0000-0003-4338-7156},
A.~Dzyuba$^{44}$\lhcborcid{0000-0003-3612-3195},
S.~Easo$^{58}$\lhcborcid{0000-0002-4027-7333},
E.~Eckstein$^{18}$\lhcborcid{0009-0009-5267-5177},
U.~Egede$^{1}$\lhcborcid{0000-0001-5493-0762},
A.~Egorychev$^{44}$\lhcborcid{0000-0001-5555-8982},
V.~Egorychev$^{44}$\lhcborcid{0000-0002-2539-673X},
S.~Eisenhardt$^{59}$\lhcborcid{0000-0002-4860-6779},
E.~Ejopu$^{63}$\lhcborcid{0000-0003-3711-7547},
L.~Eklund$^{82}$\lhcborcid{0000-0002-2014-3864},
M.~Elashri$^{66}$\lhcborcid{0000-0001-9398-953X},
J.~Ellbracht$^{19}$\lhcborcid{0000-0003-1231-6347},
S.~Ely$^{62}$\lhcborcid{0000-0003-1618-3617},
A.~Ene$^{43}$\lhcborcid{0000-0001-5513-0927},
J.~Eschle$^{69}$\lhcborcid{0000-0002-7312-3699},
S.~Esen$^{22}$\lhcborcid{0000-0003-2437-8078},
T.~Evans$^{63}$\lhcborcid{0000-0003-3016-1879},
F.~Fabiano$^{32}$\lhcborcid{0000-0001-6915-9923},
L.N.~Falcao$^{2}$\lhcborcid{0000-0003-3441-583X},
Y.~Fan$^{7}$\lhcborcid{0000-0002-3153-430X},
B.~Fang$^{7}$\lhcborcid{0000-0003-0030-3813},
L.~Fantini$^{34,q,49}$\lhcborcid{0000-0002-2351-3998},
M.~Faria$^{50}$\lhcborcid{0000-0002-4675-4209},
K.  ~Farmer$^{59}$\lhcborcid{0000-0003-2364-2877},
D.~Fazzini$^{31,o}$\lhcborcid{0000-0002-5938-4286},
L.~Felkowski$^{80}$\lhcborcid{0000-0002-0196-910X},
M.~Feng$^{5,7}$\lhcborcid{0000-0002-6308-5078},
M.~Feo$^{2}$\lhcborcid{0000-0001-5266-2442},
A.~Fernandez~Casani$^{48}$\lhcborcid{0000-0003-1394-509X},
M.~Fernandez~Gomez$^{47}$\lhcborcid{0000-0003-1984-4759},
A.D.~Fernez$^{67}$\lhcborcid{0000-0001-9900-6514},
F.~Ferrari$^{25}$\lhcborcid{0000-0002-3721-4585},
F.~Ferreira~Rodrigues$^{3}$\lhcborcid{0000-0002-4274-5583},
M.~Ferrillo$^{51}$\lhcborcid{0000-0003-1052-2198},
M.~Ferro-Luzzi$^{49}$\lhcborcid{0009-0008-1868-2165},
S.~Filippov$^{44}$\lhcborcid{0000-0003-3900-3914},
R.A.~Fini$^{24}$\lhcborcid{0000-0002-3821-3998},
M.~Fiorini$^{26,l}$\lhcborcid{0000-0001-6559-2084},
M.~Firlej$^{40}$\lhcborcid{0000-0002-1084-0084},
K.L.~Fischer$^{64}$\lhcborcid{0009-0000-8700-9910},
D.S.~Fitzgerald$^{83}$\lhcborcid{0000-0001-6862-6876},
C.~Fitzpatrick$^{63}$\lhcborcid{0000-0003-3674-0812},
T.~Fiutowski$^{40}$\lhcborcid{0000-0003-2342-8854},
F.~Fleuret$^{15}$\lhcborcid{0000-0002-2430-782X},
M.~Fontana$^{25}$\lhcborcid{0000-0003-4727-831X},
L. F. ~Foreman$^{63}$\lhcborcid{0000-0002-2741-9966},
R.~Forty$^{49}$\lhcborcid{0000-0003-2103-7577},
D.~Foulds-Holt$^{56}$\lhcborcid{0000-0001-9921-687X},
V.~Franco~Lima$^{3}$\lhcborcid{0000-0002-3761-209X},
M.~Franco~Sevilla$^{67}$\lhcborcid{0000-0002-5250-2948},
M.~Frank$^{49}$\lhcborcid{0000-0002-4625-559X},
E.~Franzoso$^{26,l}$\lhcborcid{0000-0003-2130-1593},
G.~Frau$^{63}$\lhcborcid{0000-0003-3160-482X},
C.~Frei$^{49}$\lhcborcid{0000-0001-5501-5611},
D.A.~Friday$^{63}$\lhcborcid{0000-0001-9400-3322},
J.~Fu$^{7}$\lhcborcid{0000-0003-3177-2700},
Q.~F{\"u}hring$^{19,f,56}$\lhcborcid{0000-0003-3179-2525},
Y.~Fujii$^{1}$\lhcborcid{0000-0002-0813-3065},
T.~Fulghesu$^{16}$\lhcborcid{0000-0001-9391-8619},
E.~Gabriel$^{38}$\lhcborcid{0000-0001-8300-5939},
G.~Galati$^{24}$\lhcborcid{0000-0001-7348-3312},
M.D.~Galati$^{38}$\lhcborcid{0000-0002-8716-4440},
A.~Gallas~Torreira$^{47}$\lhcborcid{0000-0002-2745-7954},
D.~Galli$^{25,j}$\lhcborcid{0000-0003-2375-6030},
S.~Gambetta$^{59}$\lhcborcid{0000-0003-2420-0501},
M.~Gandelman$^{3}$\lhcborcid{0000-0001-8192-8377},
P.~Gandini$^{30}$\lhcborcid{0000-0001-7267-6008},
B. ~Ganie$^{63}$\lhcborcid{0009-0008-7115-3940},
H.~Gao$^{7}$\lhcborcid{0000-0002-6025-6193},
R.~Gao$^{64}$\lhcborcid{0009-0004-1782-7642},
T.Q.~Gao$^{56}$\lhcborcid{0000-0001-7933-0835},
Y.~Gao$^{8}$\lhcborcid{0000-0002-6069-8995},
Y.~Gao$^{6}$\lhcborcid{0000-0003-1484-0943},
Y.~Gao$^{8}$,
L.M.~Garcia~Martin$^{50}$\lhcborcid{0000-0003-0714-8991},
P.~Garcia~Moreno$^{46}$\lhcborcid{0000-0002-3612-1651},
J.~Garc{\'\i}a~Pardi{\~n}as$^{49}$\lhcborcid{0000-0003-2316-8829},
P. ~Gardner$^{67}$\lhcborcid{0000-0002-8090-563X},
K. G. ~Garg$^{8}$\lhcborcid{0000-0002-8512-8219},
L.~Garrido$^{46}$\lhcborcid{0000-0001-8883-6539},
C.~Gaspar$^{49}$\lhcborcid{0000-0002-8009-1509},
L.L.~Gerken$^{19}$\lhcborcid{0000-0002-6769-3679},
E.~Gersabeck$^{63}$\lhcborcid{0000-0002-2860-6528},
M.~Gersabeck$^{20}$\lhcborcid{0000-0002-0075-8669},
T.~Gershon$^{57}$\lhcborcid{0000-0002-3183-5065},
S.~Ghizzo$^{29,m}$,
Z.~Ghorbanimoghaddam$^{55}$,
L.~Giambastiani$^{33,p}$\lhcborcid{0000-0002-5170-0635},
F. I.~Giasemis$^{16,e}$\lhcborcid{0000-0003-0622-1069},
V.~Gibson$^{56}$\lhcborcid{0000-0002-6661-1192},
H.K.~Giemza$^{42}$\lhcborcid{0000-0003-2597-8796},
A.L.~Gilman$^{64}$\lhcborcid{0000-0001-5934-7541},
M.~Giovannetti$^{28}$\lhcborcid{0000-0003-2135-9568},
A.~Giovent{\`u}$^{46}$\lhcborcid{0000-0001-5399-326X},
L.~Girardey$^{63}$\lhcborcid{0000-0002-8254-7274},
C.~Giugliano$^{26,l}$\lhcborcid{0000-0002-6159-4557},
M.A.~Giza$^{41}$\lhcborcid{0000-0002-0805-1561},
E.L.~Gkougkousis$^{62}$\lhcborcid{0000-0002-2132-2071},
F.C.~Glaser$^{14,22}$\lhcborcid{0000-0001-8416-5416},
V.V.~Gligorov$^{16,49}$\lhcborcid{0000-0002-8189-8267},
C.~G{\"o}bel$^{70}$\lhcborcid{0000-0003-0523-495X},
E.~Golobardes$^{45}$\lhcborcid{0000-0001-8080-0769},
D.~Golubkov$^{44}$\lhcborcid{0000-0001-6216-1596},
A.~Golutvin$^{62,49,44}$\lhcborcid{0000-0003-2500-8247},
S.~Gomez~Fernandez$^{46}$\lhcborcid{0000-0002-3064-9834},
W. ~Gomulka$^{40}$,
F.~Goncalves~Abrantes$^{64}$\lhcborcid{0000-0002-7318-482X},
M.~Goncerz$^{41}$\lhcborcid{0000-0002-9224-914X},
G.~Gong$^{4,b}$\lhcborcid{0000-0002-7822-3947},
J. A.~Gooding$^{19}$\lhcborcid{0000-0003-3353-9750},
I.V.~Gorelov$^{44}$\lhcborcid{0000-0001-5570-0133},
C.~Gotti$^{31}$\lhcborcid{0000-0003-2501-9608},
E.~Govorkova$^{65}$,
J.P.~Grabowski$^{18}$\lhcborcid{0000-0001-8461-8382},
L.A.~Granado~Cardoso$^{49}$\lhcborcid{0000-0003-2868-2173},
E.~Graug{\'e}s$^{46}$\lhcborcid{0000-0001-6571-4096},
E.~Graverini$^{50,s}$\lhcborcid{0000-0003-4647-6429},
L.~Grazette$^{57}$\lhcborcid{0000-0001-7907-4261},
G.~Graziani$^{}$\lhcborcid{0000-0001-8212-846X},
A. T.~Grecu$^{43}$\lhcborcid{0000-0002-7770-1839},
L.M.~Greeven$^{38}$\lhcborcid{0000-0001-5813-7972},
N.A.~Grieser$^{66}$\lhcborcid{0000-0003-0386-4923},
L.~Grillo$^{60}$\lhcborcid{0000-0001-5360-0091},
S.~Gromov$^{44}$\lhcborcid{0000-0002-8967-3644},
C. ~Gu$^{15}$\lhcborcid{0000-0001-5635-6063},
M.~Guarise$^{26}$\lhcborcid{0000-0001-8829-9681},
L. ~Guerry$^{11}$\lhcborcid{0009-0004-8932-4024},
V.~Guliaeva$^{44}$\lhcborcid{0000-0003-3676-5040},
P. A.~G{\"u}nther$^{22}$\lhcborcid{0000-0002-4057-4274},
A.-K.~Guseinov$^{50}$\lhcborcid{0000-0002-5115-0581},
E.~Gushchin$^{44}$\lhcborcid{0000-0001-8857-1665},
Y.~Guz$^{6,49,44}$\lhcborcid{0000-0001-7552-400X},
T.~Gys$^{49}$\lhcborcid{0000-0002-6825-6497},
K.~Habermann$^{18}$\lhcborcid{0009-0002-6342-5965},
T.~Hadavizadeh$^{1}$\lhcborcid{0000-0001-5730-8434},
C.~Hadjivasiliou$^{67}$\lhcborcid{0000-0002-2234-0001},
G.~Haefeli$^{50}$\lhcborcid{0000-0002-9257-839X},
C.~Haen$^{49}$\lhcborcid{0000-0002-4947-2928},
G. ~Hallett$^{57}$\lhcborcid{0009-0005-1427-6520},
M.M.~Halvorsen$^{49}$\lhcborcid{0000-0003-0959-3853},
P.M.~Hamilton$^{67}$\lhcborcid{0000-0002-2231-1374},
J.~Hammerich$^{61}$\lhcborcid{0000-0002-5556-1775},
Q.~Han$^{33}$\lhcborcid{0000-0002-7958-2917},
X.~Han$^{22,49}$\lhcborcid{0000-0001-7641-7505},
S.~Hansmann-Menzemer$^{22}$\lhcborcid{0000-0002-3804-8734},
L.~Hao$^{7}$\lhcborcid{0000-0001-8162-4277},
N.~Harnew$^{64}$\lhcborcid{0000-0001-9616-6651},
T. H. ~Harris$^{1}$\lhcborcid{0009-0000-1763-6759},
M.~Hartmann$^{14}$\lhcborcid{0009-0005-8756-0960},
S.~Hashmi$^{40}$\lhcborcid{0000-0003-2714-2706},
J.~He$^{7,c}$\lhcborcid{0000-0002-1465-0077},
F.~Hemmer$^{49}$\lhcborcid{0000-0001-8177-0856},
C.~Henderson$^{66}$\lhcborcid{0000-0002-6986-9404},
R.D.L.~Henderson$^{1,57}$\lhcborcid{0000-0001-6445-4907},
A.M.~Hennequin$^{49}$\lhcborcid{0009-0008-7974-3785},
K.~Hennessy$^{61}$\lhcborcid{0000-0002-1529-8087},
L.~Henry$^{50}$\lhcborcid{0000-0003-3605-832X},
J.~Herd$^{62}$\lhcborcid{0000-0001-7828-3694},
P.~Herrero~Gascon$^{22}$\lhcborcid{0000-0001-6265-8412},
J.~Heuel$^{17}$\lhcborcid{0000-0001-9384-6926},
A.~Hicheur$^{3}$\lhcborcid{0000-0002-3712-7318},
G.~Hijano~Mendizabal$^{51}$,
J.~Horswill$^{63}$\lhcborcid{0000-0002-9199-8616},
R.~Hou$^{8}$\lhcborcid{0000-0002-3139-3332},
Y.~Hou$^{11}$\lhcborcid{0000-0001-6454-278X},
N.~Howarth$^{61}$,
J.~Hu$^{72}$\lhcborcid{0000-0002-8227-4544},
W.~Hu$^{6}$\lhcborcid{0000-0002-2855-0544},
X.~Hu$^{4,b}$\lhcborcid{0000-0002-5924-2683},
W.~Huang$^{7}$\lhcborcid{0000-0002-1407-1729},
W.~Hulsbergen$^{38}$\lhcborcid{0000-0003-3018-5707},
R.J.~Hunter$^{57}$\lhcborcid{0000-0001-7894-8799},
M.~Hushchyn$^{44}$\lhcborcid{0000-0002-8894-6292},
D.~Hutchcroft$^{61}$\lhcborcid{0000-0002-4174-6509},
M.~Idzik$^{40}$\lhcborcid{0000-0001-6349-0033},
D.~Ilin$^{44}$\lhcborcid{0000-0001-8771-3115},
P.~Ilten$^{66}$\lhcborcid{0000-0001-5534-1732},
A.~Inglessi$^{44}$\lhcborcid{0000-0002-2522-6722},
A.~Iniukhin$^{44}$\lhcborcid{0000-0002-1940-6276},
A.~Ishteev$^{44}$\lhcborcid{0000-0003-1409-1428},
K.~Ivshin$^{44}$\lhcborcid{0000-0001-8403-0706},
R.~Jacobsson$^{49}$\lhcborcid{0000-0003-4971-7160},
H.~Jage$^{17}$\lhcborcid{0000-0002-8096-3792},
S.J.~Jaimes~Elles$^{75,49,48}$\lhcborcid{0000-0003-0182-8638},
S.~Jakobsen$^{49}$\lhcborcid{0000-0002-6564-040X},
E.~Jans$^{38}$\lhcborcid{0000-0002-5438-9176},
B.K.~Jashal$^{48}$\lhcborcid{0000-0002-0025-4663},
A.~Jawahery$^{67}$\lhcborcid{0000-0003-3719-119X},
V.~Jevtic$^{19,f}$\lhcborcid{0000-0001-6427-4746},
E.~Jiang$^{67}$\lhcborcid{0000-0003-1728-8525},
X.~Jiang$^{5,7}$\lhcborcid{0000-0001-8120-3296},
Y.~Jiang$^{7}$\lhcborcid{0000-0002-8964-5109},
Y. J. ~Jiang$^{6}$\lhcborcid{0000-0002-0656-8647},
M.~John$^{64}$\lhcborcid{0000-0002-8579-844X},
A. ~John~Rubesh~Rajan$^{23}$\lhcborcid{0000-0002-9850-4965},
D.~Johnson$^{54}$\lhcborcid{0000-0003-3272-6001},
C.R.~Jones$^{56}$\lhcborcid{0000-0003-1699-8816},
T.P.~Jones$^{57}$\lhcborcid{0000-0001-5706-7255},
S.~Joshi$^{42}$\lhcborcid{0000-0002-5821-1674},
B.~Jost$^{49}$\lhcborcid{0009-0005-4053-1222},
J. ~Juan~Castella$^{56}$\lhcborcid{0009-0009-5577-1308},
N.~Jurik$^{49}$\lhcborcid{0000-0002-6066-7232},
I.~Juszczak$^{41}$\lhcborcid{0000-0002-1285-3911},
D.~Kaminaris$^{50}$\lhcborcid{0000-0002-8912-4653},
S.~Kandybei$^{52}$\lhcborcid{0000-0003-3598-0427},
M. ~Kane$^{59}$\lhcborcid{ 0009-0006-5064-966X},
Y.~Kang$^{4,b}$\lhcborcid{0000-0002-6528-8178},
C.~Kar$^{11}$\lhcborcid{0000-0002-6407-6974},
M.~Karacson$^{49}$\lhcborcid{0009-0006-1867-9674},
D.~Karpenkov$^{44}$\lhcborcid{0000-0001-8686-2303},
A.~Kauniskangas$^{50}$\lhcborcid{0000-0002-4285-8027},
J.W.~Kautz$^{66}$\lhcborcid{0000-0001-8482-5576},
M.K.~Kazanecki$^{41}$,
F.~Keizer$^{49}$\lhcborcid{0000-0002-1290-6737},
M.~Kenzie$^{56}$\lhcborcid{0000-0001-7910-4109},
T.~Ketel$^{38}$\lhcborcid{0000-0002-9652-1964},
B.~Khanji$^{69}$\lhcborcid{0000-0003-3838-281X},
A.~Kharisova$^{44}$\lhcborcid{0000-0002-5291-9583},
S.~Kholodenko$^{35,49}$\lhcborcid{0000-0002-0260-6570},
G.~Khreich$^{14}$\lhcborcid{0000-0002-6520-8203},
T.~Kirn$^{17}$\lhcborcid{0000-0002-0253-8619},
V.S.~Kirsebom$^{31}$\lhcborcid{0009-0005-4421-9025},
O.~Kitouni$^{65}$\lhcborcid{0000-0001-9695-8165},
S.~Klaver$^{39}$\lhcborcid{0000-0001-7909-1272},
N.~Kleijne$^{35,r}$\lhcborcid{0000-0003-0828-0943},
K.~Klimaszewski$^{42}$\lhcborcid{0000-0003-0741-5922},
M.R.~Kmiec$^{42}$\lhcborcid{0000-0002-1821-1848},
S.~Koliiev$^{53}$\lhcborcid{0009-0002-3680-1224},
L.~Kolk$^{19}$\lhcborcid{0000-0003-2589-5130},
A.~Konoplyannikov$^{44}$\lhcborcid{0009-0005-2645-8364},
P.~Kopciewicz$^{49}$\lhcborcid{0000-0001-9092-3527},
P.~Koppenburg$^{38}$\lhcborcid{0000-0001-8614-7203},
M.~Korolev$^{44}$\lhcborcid{0000-0002-7473-2031},
I.~Kostiuk$^{38}$\lhcborcid{0000-0002-8767-7289},
O.~Kot$^{53}$,
S.~Kotriakhova$^{}$\lhcborcid{0000-0002-1495-0053},
A.~Kozachuk$^{44}$\lhcborcid{0000-0001-6805-0395},
P.~Kravchenko$^{44}$\lhcborcid{0000-0002-4036-2060},
L.~Kravchuk$^{44}$\lhcborcid{0000-0001-8631-4200},
M.~Kreps$^{57}$\lhcborcid{0000-0002-6133-486X},
P.~Krokovny$^{44}$\lhcborcid{0000-0002-1236-4667},
W.~Krupa$^{69}$\lhcborcid{0000-0002-7947-465X},
W.~Krzemien$^{42}$\lhcborcid{0000-0002-9546-358X},
O.~Kshyvanskyi$^{53}$\lhcborcid{0009-0003-6637-841X},
S.~Kubis$^{80}$\lhcborcid{0000-0001-8774-8270},
M.~Kucharczyk$^{41}$\lhcborcid{0000-0003-4688-0050},
V.~Kudryavtsev$^{44}$\lhcborcid{0009-0000-2192-995X},
E.~Kulikova$^{44}$\lhcborcid{0009-0002-8059-5325},
A.~Kupsc$^{82}$\lhcborcid{0000-0003-4937-2270},
B. K. ~Kutsenko$^{13}$\lhcborcid{0000-0002-8366-1167},
D.~Lacarrere$^{49}$\lhcborcid{0009-0005-6974-140X},
P. ~Laguarta~Gonzalez$^{46}$\lhcborcid{0009-0005-3844-0778},
A.~Lai$^{32}$\lhcborcid{0000-0003-1633-0496},
A.~Lampis$^{32}$\lhcborcid{0000-0002-5443-4870},
D.~Lancierini$^{56}$\lhcborcid{0000-0003-1587-4555},
C.~Landesa~Gomez$^{47}$\lhcborcid{0000-0001-5241-8642},
J.J.~Lane$^{1}$\lhcborcid{0000-0002-5816-9488},
R.~Lane$^{55}$\lhcborcid{0000-0002-2360-2392},
G.~Lanfranchi$^{28}$\lhcborcid{0000-0002-9467-8001},
C.~Langenbruch$^{22}$\lhcborcid{0000-0002-3454-7261},
J.~Langer$^{19}$\lhcborcid{0000-0002-0322-5550},
O.~Lantwin$^{44}$\lhcborcid{0000-0003-2384-5973},
T.~Latham$^{57}$\lhcborcid{0000-0002-7195-8537},
F.~Lazzari$^{35,s,49}$\lhcborcid{0000-0002-3151-3453},
C.~Lazzeroni$^{54}$\lhcborcid{0000-0003-4074-4787},
R.~Le~Gac$^{13}$\lhcborcid{0000-0002-7551-6971},
H. ~Lee$^{61}$\lhcborcid{0009-0003-3006-2149},
R.~Lef{\`e}vre$^{11}$\lhcborcid{0000-0002-6917-6210},
A.~Leflat$^{44}$\lhcborcid{0000-0001-9619-6666},
S.~Legotin$^{44}$\lhcborcid{0000-0003-3192-6175},
M.~Lehuraux$^{57}$\lhcborcid{0000-0001-7600-7039},
E.~Lemos~Cid$^{49}$\lhcborcid{0000-0003-3001-6268},
O.~Leroy$^{13}$\lhcborcid{0000-0002-2589-240X},
T.~Lesiak$^{41}$\lhcborcid{0000-0002-3966-2998},
E. D.~Lesser$^{49}$\lhcborcid{0000-0001-8367-8703},
B.~Leverington$^{22}$\lhcborcid{0000-0001-6640-7274},
A.~Li$^{4,b}$\lhcborcid{0000-0001-5012-6013},
C. ~Li$^{13}$\lhcborcid{0000-0002-3554-5479},
H.~Li$^{72}$\lhcborcid{0000-0002-2366-9554},
K.~Li$^{8}$\lhcborcid{0000-0002-2243-8412},
L.~Li$^{63}$\lhcborcid{0000-0003-4625-6880},
M.~Li$^{8}$,
P.~Li$^{7}$\lhcborcid{0000-0003-2740-9765},
P.-R.~Li$^{73}$\lhcborcid{0000-0002-1603-3646},
Q. ~Li$^{5,7}$\lhcborcid{0009-0004-1932-8580},
S.~Li$^{8}$\lhcborcid{0000-0001-5455-3768},
T.~Li$^{5,d}$\lhcborcid{0000-0002-5241-2555},
T.~Li$^{72}$\lhcborcid{0000-0002-5723-0961},
Y.~Li$^{8}$,
Y.~Li$^{5}$\lhcborcid{0000-0003-2043-4669},
Z.~Lian$^{4,b}$\lhcborcid{0000-0003-4602-6946},
X.~Liang$^{69}$\lhcborcid{0000-0002-5277-9103},
S.~Libralon$^{48}$\lhcborcid{0009-0002-5841-9624},
C.~Lin$^{7}$\lhcborcid{0000-0001-7587-3365},
T.~Lin$^{58}$\lhcborcid{0000-0001-6052-8243},
R.~Lindner$^{49}$\lhcborcid{0000-0002-5541-6500},
H. ~Linton$^{62}$\lhcborcid{0009-0000-3693-1972},
V.~Lisovskyi$^{50}$\lhcborcid{0000-0003-4451-214X},
R.~Litvinov$^{32,49}$\lhcborcid{0000-0002-4234-435X},
F. L. ~Liu$^{1}$\lhcborcid{0009-0002-2387-8150},
G.~Liu$^{72}$\lhcborcid{0000-0001-5961-6588},
K.~Liu$^{73}$\lhcborcid{0000-0003-4529-3356},
S.~Liu$^{5,7}$\lhcborcid{0000-0002-6919-227X},
W. ~Liu$^{8}$,
Y.~Liu$^{59}$\lhcborcid{0000-0003-3257-9240},
Y.~Liu$^{73}$,
Y. L. ~Liu$^{62}$\lhcborcid{0000-0001-9617-6067},
G.~Loachamin~Ordonez$^{70}$,
A.~Lobo~Salvia$^{46}$\lhcborcid{0000-0002-2375-9509},
A.~Loi$^{32}$\lhcborcid{0000-0003-4176-1503},
T.~Long$^{56}$\lhcborcid{0000-0001-7292-848X},
J.H.~Lopes$^{3}$\lhcborcid{0000-0003-1168-9547},
A.~Lopez~Huertas$^{46}$\lhcborcid{0000-0002-6323-5582},
S.~L{\'o}pez~Soli{\~n}o$^{47}$\lhcborcid{0000-0001-9892-5113},
Q.~Lu$^{15}$\lhcborcid{0000-0002-6598-1941},
C.~Lucarelli$^{27}$\lhcborcid{0000-0002-8196-1828},
D.~Lucchesi$^{33,p}$\lhcborcid{0000-0003-4937-7637},
M.~Lucio~Martinez$^{79}$\lhcborcid{0000-0001-6823-2607},
V.~Lukashenko$^{38,53}$\lhcborcid{0000-0002-0630-5185},
Y.~Luo$^{6}$\lhcborcid{0009-0001-8755-2937},
A.~Lupato$^{33,i}$\lhcborcid{0000-0003-0312-3914},
E.~Luppi$^{26,l}$\lhcborcid{0000-0002-1072-5633},
K.~Lynch$^{23}$\lhcborcid{0000-0002-7053-4951},
X.-R.~Lyu$^{7}$\lhcborcid{0000-0001-5689-9578},
G. M. ~Ma$^{4,b}$\lhcborcid{0000-0001-8838-5205},
S.~Maccolini$^{19}$\lhcborcid{0000-0002-9571-7535},
F.~Machefert$^{14}$\lhcborcid{0000-0002-4644-5916},
F.~Maciuc$^{43}$\lhcborcid{0000-0001-6651-9436},
B. ~Mack$^{69}$\lhcborcid{0000-0001-8323-6454},
I.~Mackay$^{64}$\lhcborcid{0000-0003-0171-7890},
L. M. ~Mackey$^{69}$\lhcborcid{0000-0002-8285-3589},
L.R.~Madhan~Mohan$^{56}$\lhcborcid{0000-0002-9390-8821},
M. J. ~Madurai$^{54}$\lhcborcid{0000-0002-6503-0759},
A.~Maevskiy$^{44}$\lhcborcid{0000-0003-1652-8005},
D.~Magdalinski$^{38}$\lhcborcid{0000-0001-6267-7314},
D.~Maisuzenko$^{44}$\lhcborcid{0000-0001-5704-3499},
J.J.~Malczewski$^{41}$\lhcborcid{0000-0003-2744-3656},
S.~Malde$^{64}$\lhcborcid{0000-0002-8179-0707},
L.~Malentacca$^{49}$\lhcborcid{0000-0001-6717-2980},
A.~Malinin$^{44}$\lhcborcid{0000-0002-3731-9977},
T.~Maltsev$^{44}$\lhcborcid{0000-0002-2120-5633},
G.~Manca$^{32,k}$\lhcborcid{0000-0003-1960-4413},
G.~Mancinelli$^{13}$\lhcborcid{0000-0003-1144-3678},
C.~Mancuso$^{30}$\lhcborcid{0000-0002-2490-435X},
R.~Manera~Escalero$^{46}$\lhcborcid{0000-0003-4981-6847},
F. M. ~Manganella$^{37}$,
D.~Manuzzi$^{25}$\lhcborcid{0000-0002-9915-6587},
D.~Marangotto$^{30,n}$\lhcborcid{0000-0001-9099-4878},
J.F.~Marchand$^{10}$\lhcborcid{0000-0002-4111-0797},
R.~Marchevski$^{50}$\lhcborcid{0000-0003-3410-0918},
U.~Marconi$^{25}$\lhcborcid{0000-0002-5055-7224},
E.~Mariani$^{16}$,
S.~Mariani$^{49}$\lhcborcid{0000-0002-7298-3101},
C.~Marin~Benito$^{46}$\lhcborcid{0000-0003-0529-6982},
J.~Marks$^{22}$\lhcborcid{0000-0002-2867-722X},
A.M.~Marshall$^{55}$\lhcborcid{0000-0002-9863-4954},
L. ~Martel$^{64}$\lhcborcid{0000-0001-8562-0038},
G.~Martelli$^{34,q}$\lhcborcid{0000-0002-6150-3168},
G.~Martellotti$^{36}$\lhcborcid{0000-0002-8663-9037},
L.~Martinazzoli$^{49}$\lhcborcid{0000-0002-8996-795X},
M.~Martinelli$^{31,o}$\lhcborcid{0000-0003-4792-9178},
D. ~Martinez~Gomez$^{78}$\lhcborcid{0009-0001-2684-9139},
D.~Martinez~Santos$^{81}$\lhcborcid{0000-0002-6438-4483},
F.~Martinez~Vidal$^{48}$\lhcborcid{0000-0001-6841-6035},
A. ~Martorell~i~Granollers$^{45}$\lhcborcid{0009-0005-6982-9006},
A.~Massafferri$^{2}$\lhcborcid{0000-0002-3264-3401},
R.~Matev$^{49}$\lhcborcid{0000-0001-8713-6119},
A.~Mathad$^{49}$\lhcborcid{0000-0002-9428-4715},
V.~Matiunin$^{44}$\lhcborcid{0000-0003-4665-5451},
C.~Matteuzzi$^{69}$\lhcborcid{0000-0002-4047-4521},
K.R.~Mattioli$^{15}$\lhcborcid{0000-0003-2222-7727},
A.~Mauri$^{62}$\lhcborcid{0000-0003-1664-8963},
E.~Maurice$^{15}$\lhcborcid{0000-0002-7366-4364},
J.~Mauricio$^{46}$\lhcborcid{0000-0002-9331-1363},
P.~Mayencourt$^{50}$\lhcborcid{0000-0002-8210-1256},
J.~Mazorra~de~Cos$^{48}$\lhcborcid{0000-0003-0525-2736},
M.~Mazurek$^{42}$\lhcborcid{0000-0002-3687-9630},
M.~McCann$^{62}$\lhcborcid{0000-0002-3038-7301},
T.H.~McGrath$^{63}$\lhcborcid{0000-0001-8993-3234},
N.T.~McHugh$^{60}$\lhcborcid{0000-0002-5477-3995},
A.~McNab$^{63}$\lhcborcid{0000-0001-5023-2086},
R.~McNulty$^{23}$\lhcborcid{0000-0001-7144-0175},
B.~Meadows$^{66}$\lhcborcid{0000-0002-1947-8034},
G.~Meier$^{19}$\lhcborcid{0000-0002-4266-1726},
D.~Melnychuk$^{42}$\lhcborcid{0000-0003-1667-7115},
F. M. ~Meng$^{4,b}$\lhcborcid{0009-0004-1533-6014},
M.~Merk$^{38,79}$\lhcborcid{0000-0003-0818-4695},
A.~Merli$^{50}$\lhcborcid{0000-0002-0374-5310},
L.~Meyer~Garcia$^{67}$\lhcborcid{0000-0002-2622-8551},
D.~Miao$^{5,7}$\lhcborcid{0000-0003-4232-5615},
H.~Miao$^{7}$\lhcborcid{0000-0002-1936-5400},
M.~Mikhasenko$^{76}$\lhcborcid{0000-0002-6969-2063},
D.A.~Milanes$^{75,x}$\lhcborcid{0000-0001-7450-1121},
A.~Minotti$^{31,o}$\lhcborcid{0000-0002-0091-5177},
E.~Minucci$^{28}$\lhcborcid{0000-0002-3972-6824},
T.~Miralles$^{11}$\lhcborcid{0000-0002-4018-1454},
B.~Mitreska$^{19}$\lhcborcid{0000-0002-1697-4999},
D.S.~Mitzel$^{19}$\lhcborcid{0000-0003-3650-2689},
A.~Modak$^{58}$\lhcborcid{0000-0003-1198-1441},
L.~Moeser$^{19}$,
R.A.~Mohammed$^{64}$\lhcborcid{0000-0002-3718-4144},
R.D.~Moise$^{17}$\lhcborcid{0000-0002-5662-8804},
S.~Mokhnenko$^{44}$\lhcborcid{0000-0002-1849-1472},
E. F.~Molina~Cardenas$^{83}$\lhcborcid{0009-0002-0674-5305},
T.~Momb{\"a}cher$^{49}$\lhcborcid{0000-0002-5612-979X},
M.~Monk$^{57,1}$\lhcborcid{0000-0003-0484-0157},
S.~Monteil$^{11}$\lhcborcid{0000-0001-5015-3353},
A.~Morcillo~Gomez$^{47}$\lhcborcid{0000-0001-9165-7080},
G.~Morello$^{28}$\lhcborcid{0000-0002-6180-3697},
M.J.~Morello$^{35,r}$\lhcborcid{0000-0003-4190-1078},
M.P.~Morgenthaler$^{22}$\lhcborcid{0000-0002-7699-5724},
J.~Moron$^{40}$\lhcborcid{0000-0002-1857-1675},
W. ~Morren$^{38}$\lhcborcid{0009-0004-1863-9344},
A.B.~Morris$^{49}$\lhcborcid{0000-0002-0832-9199},
A.G.~Morris$^{13}$\lhcborcid{0000-0001-6644-9888},
R.~Mountain$^{69}$\lhcborcid{0000-0003-1908-4219},
H.~Mu$^{4,b}$\lhcborcid{0000-0001-9720-7507},
Z. M. ~Mu$^{6}$\lhcborcid{0000-0001-9291-2231},
E.~Muhammad$^{57}$\lhcborcid{0000-0001-7413-5862},
F.~Muheim$^{59}$\lhcborcid{0000-0002-1131-8909},
M.~Mulder$^{78}$\lhcborcid{0000-0001-6867-8166},
K.~M{\"u}ller$^{51}$\lhcborcid{0000-0002-5105-1305},
F.~Mu{\~n}oz-Rojas$^{9}$\lhcborcid{0000-0002-4978-602X},
R.~Murta$^{62}$\lhcborcid{0000-0002-6915-8370},
P.~Naik$^{61}$\lhcborcid{0000-0001-6977-2971},
T.~Nakada$^{50}$\lhcborcid{0009-0000-6210-6861},
R.~Nandakumar$^{58}$\lhcborcid{0000-0002-6813-6794},
T.~Nanut$^{49}$\lhcborcid{0000-0002-5728-9867},
I.~Nasteva$^{3}$\lhcborcid{0000-0001-7115-7214},
M.~Needham$^{59}$\lhcborcid{0000-0002-8297-6714},
N.~Neri$^{30,n}$\lhcborcid{0000-0002-6106-3756},
S.~Neubert$^{18}$\lhcborcid{0000-0002-0706-1944},
N.~Neufeld$^{49}$\lhcborcid{0000-0003-2298-0102},
P.~Neustroev$^{44}$,
J.~Nicolini$^{19}$\lhcborcid{0000-0001-9034-3637},
D.~Nicotra$^{79}$\lhcborcid{0000-0001-7513-3033},
E.M.~Niel$^{49}$\lhcborcid{0000-0002-6587-4695},
N.~Nikitin$^{44}$\lhcborcid{0000-0003-0215-1091},
Q.~Niu$^{73}$,
P.~Nogarolli$^{3}$\lhcborcid{0009-0001-4635-1055},
P.~Nogga$^{18}$\lhcborcid{0009-0006-2269-4666},
C.~Normand$^{55}$\lhcborcid{0000-0001-5055-7710},
J.~Novoa~Fernandez$^{47}$\lhcborcid{0000-0002-1819-1381},
G.~Nowak$^{66}$\lhcborcid{0000-0003-4864-7164},
C.~Nunez$^{83}$\lhcborcid{0000-0002-2521-9346},
H. N. ~Nur$^{60}$\lhcborcid{0000-0002-7822-523X},
A.~Oblakowska-Mucha$^{40}$\lhcborcid{0000-0003-1328-0534},
V.~Obraztsov$^{44}$\lhcborcid{0000-0002-0994-3641},
T.~Oeser$^{17}$\lhcborcid{0000-0001-7792-4082},
S.~Okamura$^{26,l}$\lhcborcid{0000-0003-1229-3093},
A.~Okhotnikov$^{44}$,
O.~Okhrimenko$^{53}$\lhcborcid{0000-0002-0657-6962},
R.~Oldeman$^{32,k}$\lhcborcid{0000-0001-6902-0710},
F.~Oliva$^{59}$\lhcborcid{0000-0001-7025-3407},
M.~Olocco$^{19}$\lhcborcid{0000-0002-6968-1217},
C.J.G.~Onderwater$^{79}$\lhcborcid{0000-0002-2310-4166},
R.H.~O'Neil$^{49}$\lhcborcid{0000-0002-9797-8464},
D.~Osthues$^{19}$,
J.M.~Otalora~Goicochea$^{3}$\lhcborcid{0000-0002-9584-8500},
P.~Owen$^{51}$\lhcborcid{0000-0002-4161-9147},
A.~Oyanguren$^{48}$\lhcborcid{0000-0002-8240-7300},
O.~Ozcelik$^{59}$\lhcborcid{0000-0003-3227-9248},
F.~Paciolla$^{35,v}$\lhcborcid{0000-0002-6001-600X},
A. ~Padee$^{42}$\lhcborcid{0000-0002-5017-7168},
K.O.~Padeken$^{18}$\lhcborcid{0000-0001-7251-9125},
B.~Pagare$^{57}$\lhcborcid{0000-0003-3184-1622},
P.R.~Pais$^{22}$\lhcborcid{0009-0005-9758-742X},
T.~Pajero$^{49}$\lhcborcid{0000-0001-9630-2000},
A.~Palano$^{24}$\lhcborcid{0000-0002-6095-9593},
M.~Palutan$^{28}$\lhcborcid{0000-0001-7052-1360},
X. ~Pan$^{4,b}$\lhcborcid{0000-0002-7439-6621},
G.~Panshin$^{44}$\lhcborcid{0000-0001-9163-2051},
L.~Paolucci$^{57}$\lhcborcid{0000-0003-0465-2893},
A.~Papanestis$^{58,49}$\lhcborcid{0000-0002-5405-2901},
M.~Pappagallo$^{24,h}$\lhcborcid{0000-0001-7601-5602},
L.L.~Pappalardo$^{26,l}$\lhcborcid{0000-0002-0876-3163},
C.~Pappenheimer$^{66}$\lhcborcid{0000-0003-0738-3668},
C.~Parkes$^{63}$\lhcborcid{0000-0003-4174-1334},
D. ~Parmar$^{76}$\lhcborcid{0009-0004-8530-7630},
B.~Passalacqua$^{26,l}$\lhcborcid{0000-0003-3643-7469},
G.~Passaleva$^{27}$\lhcborcid{0000-0002-8077-8378},
D.~Passaro$^{35,r,49}$\lhcborcid{0000-0002-8601-2197},
A.~Pastore$^{24}$\lhcborcid{0000-0002-5024-3495},
M.~Patel$^{62}$\lhcborcid{0000-0003-3871-5602},
J.~Patoc$^{64}$\lhcborcid{0009-0000-1201-4918},
C.~Patrignani$^{25,j}$\lhcborcid{0000-0002-5882-1747},
A. ~Paul$^{69}$\lhcborcid{0009-0006-7202-0811},
C.J.~Pawley$^{79}$\lhcborcid{0000-0001-9112-3724},
A.~Pellegrino$^{38}$\lhcborcid{0000-0002-7884-345X},
J. ~Peng$^{5,7}$\lhcborcid{0009-0005-4236-4667},
M.~Pepe~Altarelli$^{28}$\lhcborcid{0000-0002-1642-4030},
S.~Perazzini$^{25}$\lhcborcid{0000-0002-1862-7122},
D.~Pereima$^{44}$\lhcborcid{0000-0002-7008-8082},
H. ~Pereira~Da~Costa$^{68}$\lhcborcid{0000-0002-3863-352X},
A.~Pereiro~Castro$^{47}$\lhcborcid{0000-0001-9721-3325},
P.~Perret$^{11}$\lhcborcid{0000-0002-5732-4343},
A. ~Perrevoort$^{78}$\lhcborcid{0000-0001-6343-447X},
A.~Perro$^{49,13}$\lhcborcid{0000-0002-1996-0496},
M.J.~Peters$^{66}$,
K.~Petridis$^{55}$\lhcborcid{0000-0001-7871-5119},
A.~Petrolini$^{29,m}$\lhcborcid{0000-0003-0222-7594},
J. P. ~Pfaller$^{66}$\lhcborcid{0009-0009-8578-3078},
H.~Pham$^{69}$\lhcborcid{0000-0003-2995-1953},
L.~Pica$^{35,r}$\lhcborcid{0000-0001-9837-6556},
M.~Piccini$^{34}$\lhcborcid{0000-0001-8659-4409},
L. ~Piccolo$^{32}$\lhcborcid{0000-0003-1896-2892},
B.~Pietrzyk$^{10}$\lhcborcid{0000-0003-1836-7233},
G.~Pietrzyk$^{14}$\lhcborcid{0000-0001-9622-820X},
R. N,~Pilato$^{61}$,
D.~Pinci$^{36}$\lhcborcid{0000-0002-7224-9708},
F.~Pisani$^{49}$\lhcborcid{0000-0002-7763-252X},
M.~Pizzichemi$^{31,o,49}$\lhcborcid{0000-0001-5189-230X},
V.~Placinta$^{43}$\lhcborcid{0000-0003-4465-2441},
M.~Plo~Casasus$^{47}$\lhcborcid{0000-0002-2289-918X},
T.~Poeschl$^{49}$\lhcborcid{0000-0003-3754-7221},
F.~Polci$^{16}$\lhcborcid{0000-0001-8058-0436},
M.~Poli~Lener$^{28}$\lhcborcid{0000-0001-7867-1232},
A.~Poluektov$^{13}$\lhcborcid{0000-0003-2222-9925},
N.~Polukhina$^{44}$\lhcborcid{0000-0001-5942-1772},
I.~Polyakov$^{44}$\lhcborcid{0000-0002-6855-7783},
E.~Polycarpo$^{3}$\lhcborcid{0000-0002-4298-5309},
S.~Ponce$^{49}$\lhcborcid{0000-0002-1476-7056},
D.~Popov$^{7}$\lhcborcid{0000-0002-8293-2922},
S.~Poslavskii$^{44}$\lhcborcid{0000-0003-3236-1452},
K.~Prasanth$^{59}$\lhcborcid{0000-0001-9923-0938},
C.~Prouve$^{81}$\lhcborcid{0000-0003-2000-6306},
D.~Provenzano$^{32,k}$\lhcborcid{0009-0005-9992-9761},
V.~Pugatch$^{53}$\lhcborcid{0000-0002-5204-9821},
G.~Punzi$^{35,s}$\lhcborcid{0000-0002-8346-9052},
S. ~Qasim$^{51}$\lhcborcid{0000-0003-4264-9724},
Q. Q. ~Qian$^{6}$\lhcborcid{0000-0001-6453-4691},
W.~Qian$^{7}$\lhcborcid{0000-0003-3932-7556},
N.~Qin$^{4,b}$\lhcborcid{0000-0001-8453-658X},
S.~Qu$^{4,b}$\lhcborcid{0000-0002-7518-0961},
R.~Quagliani$^{49}$\lhcborcid{0000-0002-3632-2453},
R.I.~Rabadan~Trejo$^{57}$\lhcborcid{0000-0002-9787-3910},
J.H.~Rademacker$^{55}$\lhcborcid{0000-0003-2599-7209},
M.~Rama$^{35}$\lhcborcid{0000-0003-3002-4719},
M. ~Ram\'{i}rez~Garc\'{i}a$^{83}$\lhcborcid{0000-0001-7956-763X},
V.~Ramos~De~Oliveira$^{70}$\lhcborcid{0000-0003-3049-7866},
M.~Ramos~Pernas$^{57}$\lhcborcid{0000-0003-1600-9432},
M.S.~Rangel$^{3}$\lhcborcid{0000-0002-8690-5198},
F.~Ratnikov$^{44}$\lhcborcid{0000-0003-0762-5583},
G.~Raven$^{39}$\lhcborcid{0000-0002-2897-5323},
M.~Rebollo~De~Miguel$^{48}$\lhcborcid{0000-0002-4522-4863},
F.~Redi$^{30,i}$\lhcborcid{0000-0001-9728-8984},
J.~Reich$^{55}$\lhcborcid{0000-0002-2657-4040},
F.~Reiss$^{20}$\lhcborcid{0000-0002-8395-7654},
Z.~Ren$^{7}$\lhcborcid{0000-0001-9974-9350},
P.K.~Resmi$^{64}$\lhcborcid{0000-0001-9025-2225},
R.~Ribatti$^{50}$\lhcborcid{0000-0003-1778-1213},
G. R. ~Ricart$^{15,12}$\lhcborcid{0000-0002-9292-2066},
D.~Riccardi$^{35,r}$\lhcborcid{0009-0009-8397-572X},
S.~Ricciardi$^{58}$\lhcborcid{0000-0002-4254-3658},
K.~Richardson$^{65}$\lhcborcid{0000-0002-6847-2835},
M.~Richardson-Slipper$^{59}$\lhcborcid{0000-0002-2752-001X},
K.~Rinnert$^{61}$\lhcborcid{0000-0001-9802-1122},
P.~Robbe$^{14,49}$\lhcborcid{0000-0002-0656-9033},
G.~Robertson$^{60}$\lhcborcid{0000-0002-7026-1383},
E.~Rodrigues$^{61}$\lhcborcid{0000-0003-2846-7625},
A.~Rodriguez~Alvarez$^{46}$,
E.~Rodriguez~Fernandez$^{47}$\lhcborcid{0000-0002-3040-065X},
J.A.~Rodriguez~Lopez$^{75}$\lhcborcid{0000-0003-1895-9319},
E.~Rodriguez~Rodriguez$^{49}$\lhcborcid{0000-0002-7973-8061},
J.~Roensch$^{19}$,
A.~Rogachev$^{44}$\lhcborcid{0000-0002-7548-6530},
A.~Rogovskiy$^{58}$\lhcborcid{0000-0002-1034-1058},
D.L.~Rolf$^{49}$\lhcborcid{0000-0001-7908-7214},
P.~Roloff$^{49}$\lhcborcid{0000-0001-7378-4350},
V.~Romanovskiy$^{66}$\lhcborcid{0000-0003-0939-4272},
A.~Romero~Vidal$^{47}$\lhcborcid{0000-0002-8830-1486},
G.~Romolini$^{26}$\lhcborcid{0000-0002-0118-4214},
F.~Ronchetti$^{50}$\lhcborcid{0000-0003-3438-9774},
T.~Rong$^{6}$\lhcborcid{0000-0002-5479-9212},
M.~Rotondo$^{28}$\lhcborcid{0000-0001-5704-6163},
S. R. ~Roy$^{22}$\lhcborcid{0000-0002-3999-6795},
M.S.~Rudolph$^{69}$\lhcborcid{0000-0002-0050-575X},
M.~Ruiz~Diaz$^{22}$\lhcborcid{0000-0001-6367-6815},
R.A.~Ruiz~Fernandez$^{47}$\lhcborcid{0000-0002-5727-4454},
J.~Ruiz~Vidal$^{82,aa}$\lhcborcid{0000-0001-8362-7164},
A.~Ryzhikov$^{44}$\lhcborcid{0000-0002-3543-0313},
J.~Ryzka$^{40}$\lhcborcid{0000-0003-4235-2445},
J. J.~Saavedra-Arias$^{9}$\lhcborcid{0000-0002-2510-8929},
J.J.~Saborido~Silva$^{47}$\lhcborcid{0000-0002-6270-130X},
R.~Sadek$^{15}$\lhcborcid{0000-0003-0438-8359},
N.~Sagidova$^{44}$\lhcborcid{0000-0002-2640-3794},
D.~Sahoo$^{77}$\lhcborcid{0000-0002-5600-9413},
N.~Sahoo$^{54}$\lhcborcid{0000-0001-9539-8370},
B.~Saitta$^{32,k}$\lhcborcid{0000-0003-3491-0232},
M.~Salomoni$^{31,49,o}$\lhcborcid{0009-0007-9229-653X},
I.~Sanderswood$^{48}$\lhcborcid{0000-0001-7731-6757},
R.~Santacesaria$^{36}$\lhcborcid{0000-0003-3826-0329},
C.~Santamarina~Rios$^{47}$\lhcborcid{0000-0002-9810-1816},
M.~Santimaria$^{28}$\lhcborcid{0000-0002-8776-6759},
L.~Santoro~$^{2}$\lhcborcid{0000-0002-2146-2648},
E.~Santovetti$^{37}$\lhcborcid{0000-0002-5605-1662},
A.~Saputi$^{26,49}$\lhcborcid{0000-0001-6067-7863},
D.~Saranin$^{44}$\lhcborcid{0000-0002-9617-9986},
A.~Sarnatskiy$^{78}$\lhcborcid{0009-0007-2159-3633},
G.~Sarpis$^{59}$\lhcborcid{0000-0003-1711-2044},
M.~Sarpis$^{63}$\lhcborcid{0000-0002-6402-1674},
C.~Satriano$^{36,t}$\lhcborcid{0000-0002-4976-0460},
A.~Satta$^{37}$\lhcborcid{0000-0003-2462-913X},
M.~Saur$^{6}$\lhcborcid{0000-0001-8752-4293},
D.~Savrina$^{44}$\lhcborcid{0000-0001-8372-6031},
H.~Sazak$^{17}$\lhcborcid{0000-0003-2689-1123},
F.~Sborzacchi$^{49,28}$\lhcborcid{0009-0004-7916-2682},
L.G.~Scantlebury~Smead$^{64}$\lhcborcid{0000-0001-8702-7991},
A.~Scarabotto$^{19}$\lhcborcid{0000-0003-2290-9672},
S.~Schael$^{17}$\lhcborcid{0000-0003-4013-3468},
S.~Scherl$^{61}$\lhcborcid{0000-0003-0528-2724},
M.~Schiller$^{60}$\lhcborcid{0000-0001-8750-863X},
H.~Schindler$^{49}$\lhcborcid{0000-0002-1468-0479},
M.~Schmelling$^{21}$\lhcborcid{0000-0003-3305-0576},
B.~Schmidt$^{49}$\lhcborcid{0000-0002-8400-1566},
S.~Schmitt$^{17}$\lhcborcid{0000-0002-6394-1081},
H.~Schmitz$^{18}$,
O.~Schneider$^{50}$\lhcborcid{0000-0002-6014-7552},
A.~Schopper$^{49}$\lhcborcid{0000-0002-8581-3312},
N.~Schulte$^{19}$\lhcborcid{0000-0003-0166-2105},
S.~Schulte$^{50}$\lhcborcid{0009-0001-8533-0783},
M.H.~Schune$^{14}$\lhcborcid{0000-0002-3648-0830},
R.~Schwemmer$^{49}$\lhcborcid{0009-0005-5265-9792},
G.~Schwering$^{17}$\lhcborcid{0000-0003-1731-7939},
B.~Sciascia$^{28}$\lhcborcid{0000-0003-0670-006X},
A.~Sciuccati$^{49}$\lhcborcid{0000-0002-8568-1487},
I.~Segal$^{76}$\lhcborcid{0000-0001-8605-3020},
S.~Sellam$^{47}$\lhcborcid{0000-0003-0383-1451},
A.~Semennikov$^{44}$\lhcborcid{0000-0003-1130-2197},
T.~Senger$^{51}$\lhcborcid{0009-0006-2212-6431},
M.~Senghi~Soares$^{39}$\lhcborcid{0000-0001-9676-6059},
A.~Sergi$^{29,m}$\lhcborcid{0000-0001-9495-6115},
N.~Serra$^{51}$\lhcborcid{0000-0002-5033-0580},
L.~Sestini$^{33}$\lhcborcid{0000-0002-1127-5144},
A.~Seuthe$^{19}$\lhcborcid{0000-0002-0736-3061},
Y.~Shang$^{6}$\lhcborcid{0000-0001-7987-7558},
D.M.~Shangase$^{83}$\lhcborcid{0000-0002-0287-6124},
M.~Shapkin$^{44}$\lhcborcid{0000-0002-4098-9592},
R. S. ~Sharma$^{69}$\lhcborcid{0000-0003-1331-1791},
I.~Shchemerov$^{44}$\lhcborcid{0000-0001-9193-8106},
L.~Shchutska$^{50}$\lhcborcid{0000-0003-0700-5448},
T.~Shears$^{61}$\lhcborcid{0000-0002-2653-1366},
L.~Shekhtman$^{44}$\lhcborcid{0000-0003-1512-9715},
Z.~Shen$^{6}$\lhcborcid{0000-0003-1391-5384},
S.~Sheng$^{5,7}$\lhcborcid{0000-0002-1050-5649},
V.~Shevchenko$^{44}$\lhcborcid{0000-0003-3171-9125},
B.~Shi$^{7}$\lhcborcid{0000-0002-5781-8933},
Q.~Shi$^{7}$\lhcborcid{0000-0001-7915-8211},
Y.~Shimizu$^{14}$\lhcborcid{0000-0002-4936-1152},
E.~Shmanin$^{25}$\lhcborcid{0000-0002-8868-1730},
R.~Shorkin$^{44}$\lhcborcid{0000-0001-8881-3943},
J.D.~Shupperd$^{69}$\lhcborcid{0009-0006-8218-2566},
R.~Silva~Coutinho$^{69}$\lhcborcid{0000-0002-1545-959X},
G.~Simi$^{33,p}$\lhcborcid{0000-0001-6741-6199},
S.~Simone$^{24,h}$\lhcborcid{0000-0003-3631-8398},
N.~Skidmore$^{57}$\lhcborcid{0000-0003-3410-0731},
T.~Skwarnicki$^{69}$\lhcborcid{0000-0002-9897-9506},
M.W.~Slater$^{54}$\lhcborcid{0000-0002-2687-1950},
J.C.~Smallwood$^{64}$\lhcborcid{0000-0003-2460-3327},
E.~Smith$^{65}$\lhcborcid{0000-0002-9740-0574},
K.~Smith$^{68}$\lhcborcid{0000-0002-1305-3377},
M.~Smith$^{62}$\lhcborcid{0000-0002-3872-1917},
A.~Snoch$^{38}$\lhcborcid{0000-0001-6431-6360},
L.~Soares~Lavra$^{59}$\lhcborcid{0000-0002-2652-123X},
M.D.~Sokoloff$^{66}$\lhcborcid{0000-0001-6181-4583},
F.J.P.~Soler$^{60}$\lhcborcid{0000-0002-4893-3729},
A.~Solomin$^{44,55}$\lhcborcid{0000-0003-0644-3227},
A.~Solovev$^{44}$\lhcborcid{0000-0002-5355-5996},
I.~Solovyev$^{44}$\lhcborcid{0000-0003-4254-6012},
N. S. ~Sommerfeld$^{18}$\lhcborcid{0009-0006-7822-2860},
R.~Song$^{1}$\lhcborcid{0000-0002-8854-8905},
Y.~Song$^{50}$\lhcborcid{0000-0003-0256-4320},
Y.~Song$^{4,b}$\lhcborcid{0000-0003-1959-5676},
Y. S. ~Song$^{6}$\lhcborcid{0000-0003-3471-1751},
F.L.~Souza~De~Almeida$^{69}$\lhcborcid{0000-0001-7181-6785},
B.~Souza~De~Paula$^{3}$\lhcborcid{0009-0003-3794-3408},
E.~Spadaro~Norella$^{29,m}$\lhcborcid{0000-0002-1111-5597},
E.~Spedicato$^{25}$\lhcborcid{0000-0002-4950-6665},
J.G.~Speer$^{19}$\lhcborcid{0000-0002-6117-7307},
E.~Spiridenkov$^{44}$,
P.~Spradlin$^{60}$\lhcborcid{0000-0002-5280-9464},
V.~Sriskaran$^{49}$\lhcborcid{0000-0002-9867-0453},
F.~Stagni$^{49}$\lhcborcid{0000-0002-7576-4019},
M.~Stahl$^{76}$\lhcborcid{0000-0001-8476-8188},
S.~Stahl$^{49}$\lhcborcid{0000-0002-8243-400X},
S.~Stanislaus$^{64}$\lhcborcid{0000-0003-1776-0498},
M. ~Stefaniak$^{84}$\lhcborcid{0000-0002-5820-1054},
E.N.~Stein$^{49}$\lhcborcid{0000-0001-5214-8865},
O.~Steinkamp$^{51}$\lhcborcid{0000-0001-7055-6467},
O.~Stenyakin$^{44}$,
H.~Stevens$^{19}$\lhcborcid{0000-0002-9474-9332},
D.~Strekalina$^{44}$\lhcborcid{0000-0003-3830-4889},
Y.~Su$^{7}$\lhcborcid{0000-0002-2739-7453},
F.~Suljik$^{64}$\lhcborcid{0000-0001-6767-7698},
J.~Sun$^{32}$\lhcborcid{0000-0002-6020-2304},
L.~Sun$^{74}$\lhcborcid{0000-0002-0034-2567},
D.~Sundfeld$^{2}$\lhcborcid{0000-0002-5147-3698},
W.~Sutcliffe$^{51}$,
P.N.~Swallow$^{54}$\lhcborcid{0000-0003-2751-8515},
K.~Swientek$^{40}$\lhcborcid{0000-0001-6086-4116},
F.~Swystun$^{56}$\lhcborcid{0009-0006-0672-7771},
A.~Szabelski$^{42}$\lhcborcid{0000-0002-6604-2938},
T.~Szumlak$^{40}$\lhcborcid{0000-0002-2562-7163},
Y.~Tan$^{4,b}$\lhcborcid{0000-0003-3860-6545},
Y.~Tang$^{74}$\lhcborcid{0000-0002-6558-6730},
M.D.~Tat$^{22}$\lhcborcid{0000-0002-6866-7085},
A.~Terentev$^{44}$\lhcborcid{0000-0003-2574-8560},
F.~Terzuoli$^{35,v,49}$\lhcborcid{0000-0002-9717-225X},
F.~Teubert$^{49}$\lhcborcid{0000-0003-3277-5268},
E.~Thomas$^{49}$\lhcborcid{0000-0003-0984-7593},
D.J.D.~Thompson$^{54}$\lhcborcid{0000-0003-1196-5943},
H.~Tilquin$^{62}$\lhcborcid{0000-0003-4735-2014},
V.~Tisserand$^{11}$\lhcborcid{0000-0003-4916-0446},
S.~T'Jampens$^{10}$\lhcborcid{0000-0003-4249-6641},
M.~Tobin$^{5,49}$\lhcborcid{0000-0002-2047-7020},
L.~Tomassetti$^{26,l}$\lhcborcid{0000-0003-4184-1335},
G.~Tonani$^{30,n}$\lhcborcid{0000-0001-7477-1148},
X.~Tong$^{6}$\lhcborcid{0000-0002-5278-1203},
T.~Tork$^{30}$,
D.~Torres~Machado$^{2}$\lhcborcid{0000-0001-7030-6468},
L.~Toscano$^{19}$\lhcborcid{0009-0007-5613-6520},
D.Y.~Tou$^{4,b}$\lhcborcid{0000-0002-4732-2408},
C.~Trippl$^{45}$\lhcborcid{0000-0003-3664-1240},
G.~Tuci$^{22}$\lhcborcid{0000-0002-0364-5758},
N.~Tuning$^{38}$\lhcborcid{0000-0003-2611-7840},
L.H.~Uecker$^{22}$\lhcborcid{0000-0003-3255-9514},
A.~Ukleja$^{40}$\lhcborcid{0000-0003-0480-4850},
D.J.~Unverzagt$^{22}$\lhcborcid{0000-0002-1484-2546},
B. ~Urbach$^{59}$\lhcborcid{0009-0001-4404-561X},
A.~Usachov$^{39}$\lhcborcid{0000-0002-5829-6284},
A.~Ustyuzhanin$^{44}$\lhcborcid{0000-0001-7865-2357},
U.~Uwer$^{22}$\lhcborcid{0000-0002-8514-3777},
V.~Vagnoni$^{25}$\lhcborcid{0000-0003-2206-311X},
V. ~Valcarce~Cadenas$^{47}$\lhcborcid{0009-0006-3241-8964},
G.~Valenti$^{25}$\lhcborcid{0000-0002-6119-7535},
N.~Valls~Canudas$^{49}$\lhcborcid{0000-0001-8748-8448},
J.~van~Eldik$^{49}$\lhcborcid{0000-0002-3221-7664},
H.~Van~Hecke$^{68}$\lhcborcid{0000-0001-7961-7190},
E.~van~Herwijnen$^{62}$\lhcborcid{0000-0001-8807-8811},
C.B.~Van~Hulse$^{47,y}$\lhcborcid{0000-0002-5397-6782},
R.~Van~Laak$^{50}$\lhcborcid{0000-0002-7738-6066},
M.~van~Veghel$^{38}$\lhcborcid{0000-0001-6178-6623},
G.~Vasquez$^{51}$\lhcborcid{0000-0002-3285-7004},
R.~Vazquez~Gomez$^{46}$\lhcborcid{0000-0001-5319-1128},
P.~Vazquez~Regueiro$^{47}$\lhcborcid{0000-0002-0767-9736},
C.~V{\'a}zquez~Sierra$^{47}$\lhcborcid{0000-0002-5865-0677},
S.~Vecchi$^{26}$\lhcborcid{0000-0002-4311-3166},
J.J.~Velthuis$^{55}$\lhcborcid{0000-0002-4649-3221},
M.~Veltri$^{27,w}$\lhcborcid{0000-0001-7917-9661},
A.~Venkateswaran$^{50}$\lhcborcid{0000-0001-6950-1477},
M.~Verdoglia$^{32}$\lhcborcid{0009-0006-3864-8365},
M.~Vesterinen$^{57}$\lhcborcid{0000-0001-7717-2765},
D. ~Vico~Benet$^{64}$\lhcborcid{0009-0009-3494-2825},
P. ~Vidrier~Villalba$^{46}$\lhcborcid{0009-0005-5503-8334},
M.~Vieites~Diaz$^{47}$\lhcborcid{0000-0002-0944-4340},
X.~Vilasis-Cardona$^{45}$\lhcborcid{0000-0002-1915-9543},
E.~Vilella~Figueras$^{61}$\lhcborcid{0000-0002-7865-2856},
A.~Villa$^{25}$\lhcborcid{0000-0002-9392-6157},
P.~Vincent$^{16}$\lhcborcid{0000-0002-9283-4541},
F.C.~Volle$^{54}$\lhcborcid{0000-0003-1828-3881},
D.~vom~Bruch$^{13}$\lhcborcid{0000-0001-9905-8031},
N.~Voropaev$^{44}$\lhcborcid{0000-0002-2100-0726},
K.~Vos$^{79}$\lhcborcid{0000-0002-4258-4062},
C.~Vrahas$^{59}$\lhcborcid{0000-0001-6104-1496},
J.~Wagner$^{19}$\lhcborcid{0000-0002-9783-5957},
J.~Walsh$^{35}$\lhcborcid{0000-0002-7235-6976},
E.J.~Walton$^{1,57}$\lhcborcid{0000-0001-6759-2504},
G.~Wan$^{6}$\lhcborcid{0000-0003-0133-1664},
C.~Wang$^{22}$\lhcborcid{0000-0002-5909-1379},
G.~Wang$^{8}$\lhcborcid{0000-0001-6041-115X},
H.~Wang$^{73}$,
J.~Wang$^{6}$\lhcborcid{0000-0001-7542-3073},
J.~Wang$^{5}$\lhcborcid{0000-0002-6391-2205},
J.~Wang$^{4,b}$\lhcborcid{0000-0002-3281-8136},
J.~Wang$^{74}$\lhcborcid{0000-0001-6711-4465},
M.~Wang$^{49}$\lhcborcid{0000-0003-4062-710X},
N. W. ~Wang$^{7}$\lhcborcid{0000-0002-6915-6607},
R.~Wang$^{55}$\lhcborcid{0000-0002-2629-4735},
X.~Wang$^{8}$,
X.~Wang$^{72}$\lhcborcid{0000-0002-2399-7646},
X. W. ~Wang$^{62}$\lhcborcid{0000-0001-9565-8312},
Y.~Wang$^{6}$\lhcborcid{0009-0003-2254-7162},
Y. W. ~Wang$^{73}$,
Z.~Wang$^{14}$\lhcborcid{0000-0002-5041-7651},
Z.~Wang$^{4,b}$\lhcborcid{0000-0003-0597-4878},
Z.~Wang$^{30}$\lhcborcid{0000-0003-4410-6889},
J.A.~Ward$^{57,1}$\lhcborcid{0000-0003-4160-9333},
M.~Waterlaat$^{49}$,
N.K.~Watson$^{54}$\lhcborcid{0000-0002-8142-4678},
D.~Websdale$^{62}$\lhcborcid{0000-0002-4113-1539},
Y.~Wei$^{6}$\lhcborcid{0000-0001-6116-3944},
J.~Wendel$^{81}$\lhcborcid{0000-0003-0652-721X},
B.D.C.~Westhenry$^{55}$\lhcborcid{0000-0002-4589-2626},
C.~White$^{56}$\lhcborcid{0009-0002-6794-9547},
M.~Whitehead$^{60}$\lhcborcid{0000-0002-2142-3673},
E.~Whiter$^{54}$\lhcborcid{0009-0003-3902-8123},
A.R.~Wiederhold$^{63}$\lhcborcid{0000-0002-1023-1086},
D.~Wiedner$^{19}$\lhcborcid{0000-0002-4149-4137},
G.~Wilkinson$^{64}$\lhcborcid{0000-0001-5255-0619},
M.K.~Wilkinson$^{66}$\lhcborcid{0000-0001-6561-2145},
M.~Williams$^{65}$\lhcborcid{0000-0001-8285-3346},
M. J.~Williams$^{49}$,
M.R.J.~Williams$^{59}$\lhcborcid{0000-0001-5448-4213},
R.~Williams$^{56}$\lhcborcid{0000-0002-2675-3567},
Z. ~Williams$^{55}$\lhcborcid{0009-0009-9224-4160},
F.F.~Wilson$^{58}$\lhcborcid{0000-0002-5552-0842},
M.~Winn$^{12}$\lhcborcid{0000-0002-2207-0101},
W.~Wislicki$^{42}$\lhcborcid{0000-0001-5765-6308},
M.~Witek$^{41}$\lhcborcid{0000-0002-8317-385X},
L.~Witola$^{22}$\lhcborcid{0000-0001-9178-9921},
G.~Wormser$^{14}$\lhcborcid{0000-0003-4077-6295},
S.A.~Wotton$^{56}$\lhcborcid{0000-0003-4543-8121},
H.~Wu$^{69}$\lhcborcid{0000-0002-9337-3476},
J.~Wu$^{8}$\lhcborcid{0000-0002-4282-0977},
X.~Wu$^{74}$\lhcborcid{0000-0002-0654-7504},
Y.~Wu$^{6}$\lhcborcid{0000-0003-3192-0486},
Z.~Wu$^{7}$\lhcborcid{0000-0001-6756-9021},
K.~Wyllie$^{49}$\lhcborcid{0000-0002-2699-2189},
S.~Xian$^{72}$,
Z.~Xiang$^{5}$\lhcborcid{0000-0002-9700-3448},
Y.~Xie$^{8}$\lhcborcid{0000-0001-5012-4069},
T. X. ~Xing$^{30}$,
A.~Xu$^{35}$\lhcborcid{0000-0002-8521-1688},
L.~Xu$^{4,b}$\lhcborcid{0000-0003-2800-1438},
L.~Xu$^{4,b}$\lhcborcid{0000-0002-0241-5184},
M.~Xu$^{57}$\lhcborcid{0000-0001-8885-565X},
Z.~Xu$^{49}$\lhcborcid{0000-0002-7531-6873},
Z.~Xu$^{7}$\lhcborcid{0000-0001-9558-1079},
Z.~Xu$^{5}$\lhcborcid{0000-0001-9602-4901},
K. ~Yang$^{62}$\lhcborcid{0000-0001-5146-7311},
S.~Yang$^{7}$\lhcborcid{0000-0003-2505-0365},
X.~Yang$^{6}$\lhcborcid{0000-0002-7481-3149},
Y.~Yang$^{29,m}$\lhcborcid{0000-0002-8917-2620},
Z.~Yang$^{6}$\lhcborcid{0000-0003-2937-9782},
V.~Yeroshenko$^{14}$\lhcborcid{0000-0002-8771-0579},
H.~Yeung$^{63}$\lhcborcid{0000-0001-9869-5290},
H.~Yin$^{8}$\lhcborcid{0000-0001-6977-8257},
X. ~Yin$^{7}$\lhcborcid{0009-0003-1647-2942},
C. Y. ~Yu$^{6}$\lhcborcid{0000-0002-4393-2567},
J.~Yu$^{71}$\lhcborcid{0000-0003-1230-3300},
X.~Yuan$^{5}$\lhcborcid{0000-0003-0468-3083},
Y~Yuan$^{5,7}$\lhcborcid{0009-0000-6595-7266},
E.~Zaffaroni$^{50}$\lhcborcid{0000-0003-1714-9218},
M.~Zavertyaev$^{21}$\lhcborcid{0000-0002-4655-715X},
M.~Zdybal$^{41}$\lhcborcid{0000-0002-1701-9619},
F.~Zenesini$^{25}$\lhcborcid{0009-0001-2039-9739},
C. ~Zeng$^{5,7}$\lhcborcid{0009-0007-8273-2692},
M.~Zeng$^{4,b}$\lhcborcid{0000-0001-9717-1751},
C.~Zhang$^{6}$\lhcborcid{0000-0002-9865-8964},
D.~Zhang$^{8}$\lhcborcid{0000-0002-8826-9113},
J.~Zhang$^{7}$\lhcborcid{0000-0001-6010-8556},
L.~Zhang$^{4,b}$\lhcborcid{0000-0003-2279-8837},
S.~Zhang$^{71}$\lhcborcid{0000-0002-9794-4088},
S.~Zhang$^{64}$\lhcborcid{0000-0002-2385-0767},
Y.~Zhang$^{6}$\lhcborcid{0000-0002-0157-188X},
Y. Z. ~Zhang$^{4,b}$\lhcborcid{0000-0001-6346-8872},
Z.~Zhang$^{4,b}$\lhcborcid{0000-0002-1630-0986},
Y.~Zhao$^{22}$\lhcborcid{0000-0002-8185-3771},
A.~Zhelezov$^{22}$\lhcborcid{0000-0002-2344-9412},
S. Z. ~Zheng$^{6}$\lhcborcid{0009-0001-4723-095X},
X. Z. ~Zheng$^{4,b}$\lhcborcid{0000-0001-7647-7110},
Y.~Zheng$^{7}$\lhcborcid{0000-0003-0322-9858},
T.~Zhou$^{6}$\lhcborcid{0000-0002-3804-9948},
X.~Zhou$^{8}$\lhcborcid{0009-0005-9485-9477},
Y.~Zhou$^{7}$\lhcborcid{0000-0003-2035-3391},
V.~Zhovkovska$^{57}$\lhcborcid{0000-0002-9812-4508},
L. Z. ~Zhu$^{7}$\lhcborcid{0000-0003-0609-6456},
X.~Zhu$^{4,b}$\lhcborcid{0000-0002-9573-4570},
X.~Zhu$^{8}$\lhcborcid{0000-0002-4485-1478},
V.~Zhukov$^{17}$\lhcborcid{0000-0003-0159-291X},
J.~Zhuo$^{48}$\lhcborcid{0000-0002-6227-3368},
Q.~Zou$^{5,7}$\lhcborcid{0000-0003-0038-5038},
D.~Zuliani$^{33,p}$\lhcborcid{0000-0002-1478-4593},
G.~Zunica$^{50}$\lhcborcid{0000-0002-5972-6290}.\bigskip

{\footnotesize \it

$^{1}$School of Physics and Astronomy, Monash University, Melbourne, Australia\\
$^{2}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$^{3}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$^{4}$Department of Engineering Physics, Tsinghua University, Beijing, China\\
$^{5}$Institute Of High Energy Physics (IHEP), Beijing, China\\
$^{6}$School of Physics State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China\\
$^{7}$University of Chinese Academy of Sciences, Beijing, China\\
$^{8}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China\\
$^{9}$Consejo Nacional de Rectores  (CONARE), San Jose, Costa Rica\\
$^{10}$Universit{\'e} Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$^{11}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$^{12}$Université Paris-Saclay, Centre d'Etudes de Saclay (CEA), IRFU, Saclay, France, Gif-Sur-Yvette, France\\
$^{13}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$^{14}$Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\\
$^{15}$Laboratoire Leprince-Ringuet, CNRS/IN2P3, Ecole Polytechnique, Institut Polytechnique de Paris, Palaiseau, France\\
$^{16}$LPNHE, Sorbonne Universit{\'e}, Paris Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3, Paris, France\\
$^{17}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$^{18}$Universit{\"a}t Bonn - Helmholtz-Institut f{\"u}r Strahlen und Kernphysik, Bonn, Germany\\
$^{19}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{20}$Physikalisches Institut, Albert-Ludwigs-Universit{\"a}t Freiburg, Freiburg, Germany\\
$^{21}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$^{22}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$^{23}$School of Physics, University College Dublin, Dublin, Ireland\\
$^{24}$INFN Sezione di Bari, Bari, Italy\\
$^{25}$INFN Sezione di Bologna, Bologna, Italy\\
$^{26}$INFN Sezione di Ferrara, Ferrara, Italy\\
$^{27}$INFN Sezione di Firenze, Firenze, Italy\\
$^{28}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{29}$INFN Sezione di Genova, Genova, Italy\\
$^{30}$INFN Sezione di Milano, Milano, Italy\\
$^{31}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$^{32}$INFN Sezione di Cagliari, Monserrato, Italy\\
$^{33}$INFN Sezione di Padova, Padova, Italy\\
$^{34}$INFN Sezione di Perugia, Perugia, Italy\\
$^{35}$INFN Sezione di Pisa, Pisa, Italy\\
$^{36}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$^{37}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$^{38}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$^{39}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$^{40}$AGH - University of Krakow, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$^{41}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$^{42}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$^{43}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$^{44}$Authors affiliated with an institute formerly covered by a cooperation agreement with CERN\\
$^{45}$DS4DS, La Salle, Universitat Ramon Llull, Barcelona, Spain\\
$^{46}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$^{47}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$^{48}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain\\
$^{49}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{50}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{51}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$^{52}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$^{53}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$^{54}$School of Physics and Astronomy, University of Birmingham, Birmingham, United Kingdom\\
$^{55}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$^{56}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{57}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{58}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{59}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{60}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{61}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{62}$Imperial College London, London, United Kingdom\\
$^{63}$Department of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{64}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$^{65}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$^{66}$University of Cincinnati, Cincinnati, OH, United States\\
$^{67}$University of Maryland, College Park, MD, United States\\
$^{68}$Los Alamos National Laboratory (LANL), Los Alamos, NM, United States\\
$^{69}$Syracuse University, Syracuse, NY, United States\\
$^{70}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{3}$\\
$^{71}$School of Physics and Electronics, Hunan University, Changsha City, China, associated to $^{8}$\\
$^{72}$Guangdong Provincial Key Laboratory of Nuclear Science, Guangdong-Hong Kong Joint Laboratory of Quantum Matter, Institute of Quantum Matter, South China Normal University, Guangzhou, China, associated to $^{4}$\\
$^{73}$Lanzhou University, Lanzhou, China, associated to $^{5}$\\
$^{74}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{4}$\\
$^{75}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{16}$\\
$^{76}$Ruhr Universitaet Bochum, Fakultaet f. Physik und Astronomie, Bochum, Germany, associated to $^{19}$\\
$^{77}$Eotvos Lorand University, Budapest, Hungary, associated to $^{49}$\\
$^{78}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{38}$\\
$^{79}$Universiteit Maastricht, Maastricht, Netherlands, associated to $^{38}$\\
$^{80}$Tadeusz Kosciuszko Cracow University of Technology, Cracow, Poland, associated to $^{41}$\\
$^{81}$Universidade da Coru{\~n}a, A Coru{\~n}a, Spain, associated to $^{45}$\\
$^{82}$Department of Physics and Astronomy, Uppsala University, Uppsala, Sweden, associated to $^{60}$\\
$^{83}$University of Michigan, Ann Arbor, MI, United States, associated to $^{69}$\\
$^{84}$Ohio State University, Columbus, United States, associated to $^{68}$\\
\bigskip
$^{a}$Centro Federal de Educac{\~a}o Tecnol{\'o}gica Celso Suckow da Fonseca, Rio De Janeiro, Brazil\\
$^{b}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$^{c}$Hangzhou Institute for Advanced Study, UCAS, Hangzhou, China\\
$^{d}$School of Physics and Electronics, Henan University , Kaifeng, China\\
$^{e}$LIP6, Sorbonne Universit{\'e}, Paris, France\\
$^{f}$Lamarr Institute for Machine Learning and Artificial Intelligence, Dortmund, Germany\\
$^{g}$Universidad Nacional Aut{\'o}noma de Honduras, Tegucigalpa, Honduras\\
$^{h}$Universit{\`a} di Bari, Bari, Italy\\
$^{i}$Universit\`{a} di Bergamo, Bergamo, Italy\\
$^{j}$Universit{\`a} di Bologna, Bologna, Italy\\
$^{k}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$^{l}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$^{m}$Universit{\`a} di Genova, Genova, Italy\\
$^{n}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$^{o}$Universit{\`a} degli Studi di Milano-Bicocca, Milano, Italy\\
$^{p}$Universit{\`a} di Padova, Padova, Italy\\
$^{q}$Universit{\`a}  di Perugia, Perugia, Italy\\
$^{r}$Scuola Normale Superiore, Pisa, Italy\\
$^{s}$Universit{\`a} di Pisa, Pisa, Italy\\
$^{t}$Universit{\`a} della Basilicata, Potenza, Italy\\
$^{u}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{v}$Universit{\`a} di Siena, Siena, Italy\\
$^{w}$Universit{\`a} di Urbino, Urbino, Italy\\
$^{x}$Universidad de Ingenier\'{i}a y Tecnolog\'{i}a (UTEC), Lima, Peru\\
$^{y}$Universidad de Alcal{\'a}, Alcal{\'a} de Henares , Spain\\
$^{z}$Facultad de Ciencias Fisicas, Madrid, Spain\\
$^{aa}$Department of Physics/Division of Particle Physics, Lund, Sweden\\
\medskip
$ ^{\dagger}$Deceased
}
\end{flushleft}

==> acknowledgements.tex <==
\section*{Acknowledgements}
%
% These Acknowledgements valid from 3-May-2019
%


 \noindent We express our gratitude to our colleagues in the CERN
 accelerator departments for the excellent performance of the LHC. We
 thank the technical and administrative staff at the LHCb
 institutes.
 We acknowledge support from CERN and from the national agencies:
 ARC (Australia);
 CAPES, CNPq, FAPERJ and FINEP (Brazil); 
 MOST and NSFC (China); 
 CNRS/IN2P3 (France); 
 BMBF, DFG and MPG (Germany); 
 INFN (Italy); 
 NWO (Netherlands); 
 MNiSW and NCN (Poland); 
 MCID/IFA (Romania); 
 %MSHE (Russia); 
 MICIU and AEI (Spain);
 SNSF and SER (Switzerland); 
 NASU (Ukraine); 
 STFC (United Kingdom); 
 DOE NP and NSF (USA).
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 We acknowledge the computing resources that are provided by ARDC (Australia), 
 CBPF (Brazil),
 CERN, 
 IHEP and LZU (China),
 IN2P3 (France), 
 KIT and DESY (Germany), 
 INFN (Italy), 
 SURF (Netherlands),
 Polish WLCG (Poland),
 IFIN-HH (Romania), 
 %RRCKI and Yandex LLC (Russia), 
 PIC (Spain), CSCS (Switzerland), 
 and GridPP (United Kingdom).
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 We are indebted to the communities behind the multiple open-source
 software packages on which we depend.
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Individual groups or members have received support from
 %ARC and ARDC (Australia); % moved to national 16/01
 Key Research Program of Frontier Sciences of CAS, CAS PIFI, CAS CCEPP, 
 Fundamental Research Funds for the Central Universities,  and Sci.\ \& Tech.\ Program of Guangzhou (China);
 Minciencias (Colombia);
 EPLANET, Marie Sk\l{}odowska-Curie Actions, ERC and NextGenerationEU (European Union);
 A*MIDEX, ANR, IPhU and Labex P2IO, and R\'{e}gion Auvergne-Rh\^{o}ne-Alpes (France);
 %RFBR, RSF and Yandex LLC (Russia);
 Alexander-von-Humboldt Foundation (Germany);
 ICSC (Italy); 
 GVA, XuntaGal, GENCAT, Inditex, InTalent and Prog.~Atracci\'on Talento, CM (Spain);
 Severo Ochoa and Mar\'ia de Maeztu Units of Excellence, GVA, XuntaGal, GENCAT, InTalent-Inditex and Prog.~Atracci\'on Talento CM (Spain);
 SRC (Sweden);
 the Leverhulme Trust, the Royal Society and UKRI (United Kingdom).


\indent

Data associated to the plots in this publication as well as
in supplementary materials are made available on the
CERN document server in Ref.~\cite{cds_article}.




